Learning Optimal Deterministic Policies with Stochastic Policy Gradients

Policy gradient (PG) methods are successful approaches to deal with continuous reinforcement learning (RL) problems. They learn stochastic parametric (hyper)policies by either exploring in the space of actions or in the space of parameters. Stochastic controllers, however, are often undesirable from a practical perspective because of their lack of robustness, safety, and traceability. In common practice, stochastic (hyper)policies are learned only to deploy their deterministic version. In this paper, we make a step towards the theoretical understanding of this practice. After introducing a novel framework for modeling this scenario, we study the global convergence to the best deterministic policy, under (weak) gradient domination assumptions. Then, we illustrate how to tune the exploration level used for learning to optimize the trade-off between the sample complexity and the performance of the deployed deterministic policy. Finally, we quantitatively compare action-based and parameter-based exploration, giving a formal guise to intuitive results.

==> apx/schifezze.tex <==
\begin{proof}
	Before starting the proof, we need a preliminary result that easily follows from Theorem~\ref{thr:Jp_weak_gradient_domination}, for which it holds that:
	\begin{align*}
		\Jp(\vtheta^*_{\text{P}}) - \Jp(\vtheta) \leq \alpha \| \nabla_{\vtheta} \Jp(\vtheta) \|_2 + \alpha L_2 \psigma \sqrt{\dt} + 3 L_J \psigma \sqrt{\dt}.
	\end{align*}
	
	This result can be rewritten as:
	\begin{align*}
		\frac{1}{\alpha} \left(\Jp(\vtheta^*_{\text{P}}) - \Jp(\vtheta)\right) \leq \| \nabla_{\vtheta} \Jp(\vtheta) \|_2 +  L_2 \psigma \sqrt{\dt} + \frac{3 L_J \psigma \sqrt{\dt}}{\alpha}.
	\end{align*}
	
	For what follows, we use the following additional notation $\epsilon' = L_2 \psigma \sqrt{\dt} +  \frac{3 L_J \psigma \sqrt{\dt}}{\alpha}$ and $\mu = \frac{1}{2 \alpha^2}$.
	
	From such a result, we can write the following bound:
	\begin{align}
		\| \nabla_{\vtheta} \Jp(\vtheta) \|_2^2 \geq 	\mu \left(\Jp(\vtheta^*_{\text{P}}) - \Jp(\vtheta)\right)^2 - (\epsilon')^2. \label{eq:pgpe_fast_eq_1}
	\end{align}
	
	Considering a $k \in \dsb{K}$ it follows that:
	\begin{align*}
		\Jp(\vtheta^*_{\text{P}}) - \Jp(\vtheta_{k+1}) &= \Jp(\vtheta^*_{\text{P}}) - \Jp(\vtheta_{k+1}) + \Jp(\vtheta_{k}) - \Jp(\vtheta_{k}) \\
		&=  \Jp(\vtheta^*_{\text{P}}) - \Jp(\vtheta_{k}) - ( \Jp(\vtheta_{k+1}) - \Jp(\vtheta_{k})) \\
		&\leq \Jp(\vtheta^*_{\text{P}}) - \Jp(\vtheta_{k}) - \left<  \vtheta_{k+1} - \vtheta_{k}; \nabla_{\vtheta}\Jp(\vtheta_{k}) \right> + \frac{\Lp}{2} \|  \vtheta_{k+1} - \vtheta_{k} \|_2^2 \\
		&\leq \Jp(\vtheta^*_{\text{P}}) - \Jp(\vtheta_{k}) - \zeta_k \left< \widehat{\nabla}_{\vtheta}\Jp(\vtheta_{k})  ; \nabla_{\vtheta}\Jp(\vtheta_{k}) \right> + \frac{\Lp}{2} \zeta_k^2 \|  \widehat{\nabla}_{\vtheta}\Jp(\vtheta_{k}) \|_2^2,
	\end{align*}
	
	where the last two lines follow from the Assumption~\ref{ass:Jd_lip} and the fact that the parameter update is:
	\begin{align*}
		\vtheta_{k+1} \leftarrow \vtheta_{k} + \zeta_k \widehat{\nabla}_{\vtheta} \Jp(\vtheta_{k}).
	\end{align*}
	
	Now, we can consider the conditional expectation on $\vtheta_{k}$, for $k \in \dsb{K}$:
	\begin{align*}
		\E_k \left[ 	\Jp(\vtheta^*_{\text{P}}) - \Jp(\vtheta_{k+1}) \right] &\leq \E_k \left[ \Jp(\vtheta^*_{\text{P}}) - \Jp(\vtheta_{k}) - \zeta_k \left< \widehat{\nabla}_{\vtheta}\Jp(\vtheta_{k})  ; \nabla_{\vtheta}\Jp(\vtheta_{k}) \right> + \frac{\Lp}{2} \zeta_k^2 \|  \widehat{\nabla}_{\vtheta}\Jp(\vtheta_{k}) \|_2^2 \right] \\
		&\leq \Jp(\vtheta^*_{\text{P}}) - \Jp(\vtheta_{k}) - \zeta_k \| \nabla_{\vtheta} \Jp(\vtheta_{k}) \|_2^2+ \frac{\Lp}{2} \zeta_k^2 \E_k \left[\|  \widehat{\nabla}_{\vtheta}\Jp(\vtheta_{k}) \|_2^2\right] \\
		&\leq \Jp(\vtheta^*_{\text{P}}) - \Jp(\vtheta_{k}) - \zeta_k \left(1 -  \frac{\Lp}{2} \zeta_k \right)  \| \nabla_{\vtheta} \Jp(\vtheta_{k}) \|_2^2 + \frac{\Lp}{2} \zeta_k^2 \Var\left( \widehat{\nabla}_{\vtheta}\Jp(\vtheta_{k}) \right) \\
		&\leq \Jp(\vtheta^*_{\text{P}}) - \Jp(\vtheta_{k}) - \zeta_k \left( 1 - \frac{\Lp}{2} \zeta_k \right)  \| \nabla_{\vtheta} \Jp(\vtheta_{k}) \|_2^2 + \frac{\Lp \Vp}{2N} \zeta_k^2.
	\end{align*}

	The last derivation simply follows from the fact that $\widehat{\nabla}_{\vtheta} \Jp(\vtheta)$ is an unbiased estimator, and from the definition of $\Var(\widehat{\nabla} \Jp(\vtheta))$.
	
	Now, selecting a step size $\zeta_k \leq \frac{1}{\Lp}$, we can use the bound derived in Line~(\ref{eq:pgpe_fast_eq_1}):
	\begin{align*}
			\E_k &\left[ \Jp(\vtheta^*_{\text{P}}) - \Jp(\vtheta_{k+1}) \right] \\
			&\leq \Jp(\vtheta^*_{\text{P}}) - \Jp(\vtheta_{k}) - \zeta_k \left( 1 - \frac{\Lp}{2} \zeta_k \right) \left( \mu \left(\Jp(\vtheta^*_{\text{P}}) - \Jp(\vtheta_{k})\right)^2 - (\epsilon')^2 \right) + \frac{\Lp \Vp}{2N} \zeta_k^2 \\
			&\leq \Jp(\vtheta^*_{\text{P}}) - \Jp(\vtheta_{k}) - \mu \zeta_k \left( 1 - \frac{\Lp}{2} \zeta_k \right) \left( \Jp(\vtheta^*_{\text{P}}) - \Jp(\vtheta_{k}) \right)^2 +  \zeta_k \left( 1 - \frac{\Lp}{2} \zeta_k \right) (\epsilon')^2 + \frac{\Lp \Vp}{2N} \zeta_k^2.
	\end{align*}

	The next step is to consider the total expectation over both the terms of the inequality.
	In particular, we define: $r_k \coloneqq \E \left[\Jp(\vtheta^*_{\text{P}}) - \Jp(\vtheta_{k})\right]$.
	Having said this, we can proceed as follows:
	\begin{align*}
		r_{k+1} \leq r_k - \mu \zeta_k \left( 1 - \frac{\Lp}{2} \zeta_k \right) r_k^2 +  \zeta_k \left( 1 - \frac{\Lp}{2} \zeta_k \right) (\epsilon')^2 + \frac{\Lp \Vp}{2N} \zeta_k^2.
	\end{align*}

	If $\exists \overbar{k} \in \dsb{K}$ such that $r_{\overbar{k}} < \delta$, we are done.
	Otherwise, if $\forall k \in \dsb{K}$ it results that $r_k \geq \delta$, we can proceed as follows:
	\begin{align}
			r_{k+1} &\leq r_k - \mu \zeta_k \delta \left( 1 - \frac{\Lp}{2} \zeta_k \right) r_k +  \zeta_k \left( 1 - \frac{\Lp}{2} \zeta_k \right) (\epsilon')^2 + \frac{\Lp \Vp}{2N} \zeta_k^2 \nonumber \\
			&\leq \left( 1 - \mu \zeta_k \delta \left( 1 - \frac{\Lp}{2} \zeta_k \right)  \right) r_k +  \zeta_k \left( 1 - \frac{\Lp}{2} \zeta_k \right) (\epsilon')^2 + \frac{\Lp \Vp}{2N} \zeta_k^2 \nonumber \\
			&\leq  \left( 1 - \frac{\mu \delta \zeta_k}{2}  \right) r_k +  \zeta_k \left( 1 - \frac{\Lp}{2} \zeta_k \right) (\epsilon')^2 + \frac{\Lp \Vp}{2N} \zeta_k^2, \label{eq:pgpe_fast_eq_2}
	\end{align}
	where the last line follows because we selected $\zeta_k \leq \frac{1}{\Lp}$.
	
	For what follows, it is worth noting that $1 - \mu \delta \zeta_k \geq 0$ for $\zeta_k \leq \frac{1}{b}$ with $b \geq \mu \delta$, thus, we need to consider two different cases.
	
	\textbf{Case $K \leq \frac{b}{\mu \delta}$} We can set $\zeta_k = \frac{1}{b}$, and thus we can derive what follows:
	\begin{align}
		r_K &\leq \left( 1 - \frac{\mu \delta}{2b} \right) r_{K-1} + \frac{2b - \Lp}{2 b^2} (\epsilon')^2 + \frac{\Lp \Vp}{2 N b^2} \nonumber\\
		&\leq \left( 1 - \frac{\mu \delta}{2b} \right)^K r_{0} + \left(  \frac{2b - \Lp}{2 b^2} (\epsilon')^2 + \frac{\Lp \Vp}{2 N b^2} \right) \sum_{i=0}^{K-1} \left(1 - \frac{\mu \delta}{2b}\right)^i \nonumber\\
		&\leq  \left( 1 - \frac{\mu \delta}{2b} \right)^K r_0 +  \frac{2b - \Lp}{\mu \delta b} (\epsilon')^2 + \frac{\Lp \Vp}{N \mu \delta b} \nonumber\\
		&\leq  \left( 1 - \frac{\mu \delta}{2b} \right)^K r_0 +  \frac{2b - \Lp}{\mu^2 \delta^2 K} (\epsilon')^2 + \frac{\Lp \Vp}{N \mu^2 \delta^2 K}. \label{eq:pgpe_fast_eq_3}
	\end{align}
	
	\textbf{Case $K \geq \frac{b}{\mu \delta}$}. In such a case, it does not suffice to perform the recursion of line~(\ref{eq:pgpe_fast_eq_2}) and then apply a bound on the $K$ to highlight the dependence on the number of iterations itself.
	It is useful to define the quantity:
	\begin{align*}
		k_0 \coloneqq \left[\frac{K}{2}\right] \geq \frac{K-1}{2}.
	\end{align*}
	
	Now we can think of two cases: the one in which $k \leq k_0$ and the one in which $k > k_0$.

	When $k \leq k_0$, we can resume from line~(\ref{eq:pgpe_fast_eq_2}) and perform a derivation similar to the case in which $K \leq \frac{b}{\mu \delta}$. 
	This will provide us a bound on the quantity $r_{k_0}$ which will be useful later on.
	Setting $\zeta_k = \frac{1}{b}$ with $b \geq \mu \delta$, we can easily obtain:
	\begin{align}
		r_{k_0} &\leq \left(1 - \frac{\mu \delta}{2 b}\right)^{k_0} r_0 + \frac{2b - \Lp}{\mu \delta b} (\epsilon')^2 + \frac{\Lp \Vp}{N \mu \delta b} \nonumber \\
		&=\left(1 - \frac{\mu \delta}{2 b}\right)^{\left[\frac{K}{2}\right]} r_0 + \frac{2b - \Lp}{\mu \delta b} (\epsilon')^2 + \frac{\Lp \Vp}{N \mu \delta b}.  \label{eq:pgpe_fast_eq_4}
	\end{align}
	
	When $k > k_0$, we need to select an adaptive learning rate as:
	\begin{align*}
		\zeta_k = \frac{4}{\mu \delta \left(\frac{2b}{\mu \delta} + k - k_0\right)}.
	\end{align*}
	
	Now, we can resume form line~(\ref{eq:pgpe_fast_eq_2}) as follows:
	\begin{align*}
		r_{k} &\leq \left(1 - \frac{\mu \delta \zeta_k}{2}\right) r_{k-1} + \zeta_k \left( 1 - \frac{\Lp}{2} \zeta_k \right) (\epsilon')^2 + \frac{\Lp \Vp}{2N} \zeta_k^2 \\
		&\leq \frac{\frac{2b}{\mu \delta} + k - k_0 - 2 }{\frac{2b}{\mu \delta} + k - k_0} r_{k-1} + \frac{4 \mu \delta \left(\frac{2b}{\mu \delta} + k - k_0 \right) - 16 \Lp}{\mu^2 \delta^2} (\epsilon')^2 + \frac{8 \Lp \Vp}{N \mu^2 \delta^2 \left(\frac{2b}{\mu \delta} + k - k_0 \right)^2}. 
	\end{align*}
	
	We now need to define $w_k \coloneqq \left(\frac{2b}{\mu \delta} + k - k_0 \right)^2$.
	Then, multiplying both sides of the inequality by $w_k$, we obtain:
	\begin{align*}
		w_k r_k &\leq \left(\frac{2b}{\mu \delta} + k - k_0 \right) \left(\frac{2b}{\mu \delta} + k - k_0 - 2\right) r_{k-1} + 	\frac{4}{\mu \delta} \left(\frac{2b - 4 \Lp}{\mu \delta} + k - k_0 \right) (\epsilon')^2 + \frac{8\Lp \Vp}{N \mu^2 \delta^2} \\
		&= \left(\frac{2b}{\mu \delta} + k - k_0 - 1 \right)^2 r_{k-1} + \frac{4}{\mu \delta} \left(\frac{2b - 4 \Lp}{\mu 	\delta} + k - k_0 \right) (\epsilon')^2 + \frac{8\Lp \Vp}{N \mu^2 \delta^2} \\
		&= w_{k-1} r_{k-1} + \frac{4}{\mu \delta} \left(\frac{2b - 4 \Lp}{\mu \delta} + k - k_0 \right) (\epsilon')^2 + 	\frac{8\Lp \Vp}{N \mu^2 \delta^2}.
	\end{align*}
	
	We can telescope from $k_0$ to $K$ the terms on both sides of the last obtained inequality, obtaining what follows:
	\begin{align*}
		w_K r_K &\leq w_{k_0} r_{k_0} + \frac{4}{\mu \delta} (\epsilon')^2 \sum_{i=k_0+1}^{K} \left( \frac{2b - 4 \Lp}{\mu \delta} + k - k_0 \right) + \frac{8\Lp \Vp}{N \mu^2 \delta^2} (K - k_0) \\
		&= \frac{4b^2}{\mu^2 \delta^2} r_{k_0} + \frac{4 (2b - 4 \Lp)}{\mu^2 \delta^2} (K - k_0) (\epsilon')^2 + \frac{2 (\epsilon')^2}{\mu \delta} (K - k_0) (K - k_0 + 1) + \frac{8\Lp \Vp}{N \mu^2 \delta^2} (K - k_0).
	\end{align*}
	
	To continue the derivation, we divide both sides of the inequality by $w_K$. 
	Moreover, we use the fact that $w_K \geq (K - k_0)^2$ and the fact that $K - k_0 \geq \frac{K}{2}$.
	Thus, we can write:
	\begin{align*}
		 r_K &\leq  \frac{4b^2}{\mu^2 \delta^2 w_K} r_{k_0} + \frac{4 (2b - 4 \Lp)}{\mu^2 \delta^2 w_K} (K - k_0) (\epsilon')^2 + \frac{2 (\epsilon')^2}{\mu \delta w_K} (K - k_0) (K - k_0 + 1) + \frac{8\Lp \Vp}{N \mu^2 \delta^2 w_K} (K - k_0) \\
		 &\leq \frac{16b^2}{\mu^2 \delta^2 K^2} r_{k_0} + \frac{4 (2b - 4 \Lp)}{\mu^2 \delta^2 (K- k_0)} (\epsilon')^2 + \frac{4 (\epsilon')^2}{\mu \delta} + \frac{8\Lp \Vp}{N \mu^2 \delta^2 (K-k_0)} \\
		 &\leq \frac{16b^2}{\mu^2 \delta^2 K^2} r_{k_0} + \frac{8 (2b - 4 \Lp)}{\mu^2 \delta^2 K} (\epsilon')^2 + \frac{4 \epsilon'}{\mu} + \frac{16\Lp \Vp}{N \mu^2 \delta^2 K},
	\end{align*}
	where the last step is possible due to the fact that $\frac{(\epsilon')^2}{\delta} = \epsilon'$.
	
	Finally, by employing the bound for $r_{k_0}$ obtained in line~(\ref{eq:pgpe_fast_eq_4}) we can conclude the derivation as:
	\begin{align}
		r_K &\leq \frac{16b^2}{\mu^2 \delta^2 K^2} \left( \left(1 - \frac{\mu \delta}{2 b}\right)^{\left[\frac{K}{2}\right]} r_0 + \frac{2b - \Lp}{\mu \delta b} (\epsilon')^2 + \frac{\Lp \Vp}{N \mu \delta b} \right) + \frac{8 (2b - 4 \Lp)}{\mu^2 \delta^2 K} (\epsilon')^2 + \frac{4 \epsilon'}{\mu} + \frac{16\Lp \Vp}{N \mu^2 \delta^2 K} \nonumber \\
		&\leq 16  \left(1 - \frac{\mu \delta}{2 b}\right)^{\left[\frac{K}{2}\right]} r_0 + \frac{24 (2b - \Lp)}{\mu^2 \delta^2 K} (\epsilon')^2 + \frac{32 \Lp \Vp}{N \mu^2 \delta^2 K} + \frac{4 \epsilon'}{\mu}. \label{eq:pgpe_fast_eq_5}
	\end{align}
	where we used the fact that we are considering the case in which $K \geq \frac{b}{\mu \delta}$.
	
	In order to fully conclude the proof, we need to take the maximum between the two bounds found for $K \leq \frac{b}{\mu \delta}$ and for $K \geq \frac{b}{\mu \delta}$, with $b = \max \left\{ \Lp, \mu \delta\right\}$.
	In addition, we need to add the correction terms to pass from the $\Jp$ to the $\Jd$ domain, as shown in Lemma~\ref{lem:bound_difference_Jd_and_Jp}.
	
	All in all, we need to consider the maximum bound between the one shown in line~(\ref{eq:pgpe_fast_eq_3}) and the one shown in line~(\ref{eq:pgpe_fast_eq_5}).
	So, we can conclude the proof by saying that:
	\begin{align*}
		&\Jd(\vtheta^*) - \E \left[\Jd(\vtheta_{k})\right] \leq \\ 
        &16 \left(1 - \frac{\mu \delta}{2 b}\right)^{\left[\frac{K}{2}\right]} (\Jd(\vtheta^*) - \Jd(\vtheta_{0})) + \frac{24 (2b - \Lp)}{\mu^2 \delta^2 K} (\epsilon')^2 + \frac{32 \Lp \Vp}{N \mu^2 \delta^2 K} + \frac{4 \epsilon'}{\mu} + c(\psigma, K),
	\end{align*}
	
	where $c(\psigma, K) \coloneqq 3L_J\psigma\sqrt{\dt} + 32L_J\psigma\sqrt{\dt}  \left(1 - \frac{\mu \delta}{2 b}\right)^{\left[\frac{K}{2}\right]}$.
\end{proof}

\section{Comments on the Sample Complexity} \label{apx:sample_complexity_comments}

\subsection{PGPE Sample Complexity} \label{apx:sample_complexity_comments:pgpe}
From Theorem~\ref{thr:pgpe_fast_global_convergence} it emerges that the dominant term in the upper bound of $\Jd(\vtheta^*) - \E\left[\Jd(\vtheta_{K})\right]$ is:
\begin{align*}
	\mathcal{X} = \frac{32 \Lp \Vp}{N \mu^2 \delta^2 K} + \frac{4 \epsilon'}{\mu} + 3L_J\psigma\sqrt{\dt}.
\end{align*}

In particular:
\begin{itemize}
	\item $\epsilon' = L_2 \psigma \sqrt{\dt} + \frac{3 L_J \psigma \sqrt{\dt}}{\alpha}$, thus it is $O(\psigma)$;
	\item $\Lp = \min \left\{L_2, \frac{r^+ (1-\gamma^T)}{1-\gamma} \left(\xi_1 + \xi_2\right)\right\}$, due to Lemma~\ref{lem:Jp_bounded_hessian} and when we are dealing with a gaussian hyperpolicy, it holds that $\Lp = \min \left\{L_2, \frac{r^+ (1-\gamma^T)}{1-\gamma} \left(\psigma^{-4} + \psigma^{-2} \right)\right\}$ (the reason is explained right after this list);
	\item when dealing with a Gaussian hyperpolicy, the bound on the variance of the gradient estimator is $O(\psigma^{-2})$;
	\item $\mu$ is a constant term, since it is defined as $\mu = \frac{1}{2 \alpha^2}$.
\end{itemize}

In order to find the sample complexity, we need to find the value for $\psigma$ minimizing the $\mathcal{X}$ term.

To derive such a value of $\psigma$  we should consider both the cases in which $\Lp$ depends or not on $\psigma$ itself.

\subsubsection{Case $\Lp = L_2$}
When this is the case, it holds that:
\begin{align*}
	\mathcal{X} = O \left( \frac{1}{K \psigma^4}  + \psigma \right),
\end{align*}
thus, if we differentiate \wrt $\psigma$ we obtain what follows:
\begin{align*}
	\frac{\partial \mathcal{X}}{\partial \psigma} = 1 - \frac{4}{K \psigma^5}.
\end{align*}
We can conclude that $\psigma^* = O(K^{-1/5})$.

\subsubsection{Case $\Lp = \frac{r^+(1-\gamma^T)}{1-\gamma} \left(\xi_1 + \xi_2\right)$}
When we deal with a gaussian hyperpolicy $\nu_{\vtheta}$, where $\vtheta$ is indicating the vector of the means of the gaussian distributions associated with each dimension of the policy parameters, while the standard deviations are fixed to be $\psigma$, we know that:
\begin{align*}
	&\nabla_{\vtheta} \log \nu_{\vtheta} (\vtheta') = \frac{\vtheta' - \vtheta}{\psigma^2}, \\
	&\nabla_{\vtheta}^2 \log \nu_{\vtheta} (\vtheta') = -\frac{1}{\psigma^2}.
\end{align*}

Thus, it immediately follows that:
\begin{align*}
	&\E_{\vtheta' \sim \nu_{\vtheta}} \left[ \left\| \nabla_{\vtheta} \log \nu_{\vtheta} (\vtheta') \right\|_2^2 \right]= \E_{\vtheta' \sim \nu_{\vtheta}} \left[\frac{(\vtheta' - \vtheta)^2}{\psigma^4}\right] = \frac{1}{\psigma^2}, \\
	&\E_{\vtheta' \sim \nu_{\vtheta}} \left[\left\| \nabla_{\vtheta}^2 \log \nu_{\vtheta} (\vtheta') \right\|_2 \right] = \frac{1}{\psigma^2}.
\end{align*}

Form this fact, we can conclude that:
\begin{align*}
	\xi_1 + \xi_2 = O\left( \frac{1}{\psigma^2} \right).
\end{align*}

From this fact, the dominant complexity term is:
\begin{align*}
	\mathcal{X} = O \left( \frac{1}{K \psigma^6} + \psigma \right).
\end{align*}

For what previously shown, we can say that $\psigma^* = O(K^{-1/7})$.

\subsubsection{Conclusions}
If we aim at guaranteeing that  $\Jd(\vtheta^*) - \E\left[\Jd(\vtheta_{K})\right] \leq \epsilon$, in the case in which we deal with a gaussian hyperpolicy $\nu_{\vtheta}$, we need to select a number of iteration that is:
\begin{itemize}[noitemsep, leftmargin=*, topsep=-2pt]
	\item if $\Lp = L_2$, then $K = O(\epsilon^{-5})$;
	\item if $\Lp = \frac{r^+(1-\gamma^T)}{1-\gamma} \left(\xi_1 + \xi_2\right)$, then $K = O(\epsilon^{-7})$.
\end{itemize}

Moreover, we can notice is that $\psigma \approx \epsilon$, in order to guarantee to converge to the global optimum of the underlying deterministic policy class.

Finally, notice that the relevant case is obtained when $\psigma \xrightarrow[]{} 0$, thus when $\Lp = L_2$.

\begin{lemma} \label{lem:bound_difference_Jd_and_Ja}
    Under Assumption~\ref{ass:lipMdp}, $\forall \vtheta \in \Theta$ it holds that:
    \begin{align*}
        \left| \Jd(\vtheta) - \Ja(\vtheta) \right| \leq \left( \frac{\gamma + \gamma^{1 + T} (T-1) - T \gamma^T }{(1-\gamma)^2} L_{\log p}  R_{\max} + \frac{1 - \gamma^T}{1 - \gamma} L_r \right) \asigma \sqrt{\da}.
    \end{align*}
\end{lemma}
\begin{proof}
    In AB exploration, at each step the action suggested by $\mu_{\vtheta}$ is perturbed by a certain amount of noise.
    Thus, at the $t$-th step the action suggested by $\va_{t} \sim \pi_{\vtheta}(\cdot | \vs_{t})$ is $\mu_{\vtheta}(\vs_{t}) + \underline{\vepsilon}_{t}$, with $\underline{\vepsilon}_{t} \sim \mathcal{N}(\bm{0}_{\dt}, \asigma I_{\dt})$.
    \todomp{non $d_{\mathcal{A}}$?}

    For what follows, we consider $\underline{\vepsilon}$ as a $T$-dimensional vector of noises, one for each step in a trajectory $\tau$. More formally, we have that: $\underline{\vepsilon} \coloneqq (\underline{\vepsilon}_{0}, ..., \underline{\vepsilon}_{T-1})^{\top}$.
    Note that each noise vector $\underline{\vepsilon}_{t}$ is $\da$-dimensional.
    
    Moreover, with a slight abuse of notation, we indicate as $\mu_{\vtheta} + \underline{\vepsilon}$ a policy adding at each time step $t$ the corresponding noise element $\underline{\vepsilon}_{t}$ to the action selected by the deterministic policy $\mu_{\vtheta}$.
    
    Given such a notation, and considering a generic parametric configuration $\vtheta \in \Theta$, we can write the AB performance index $\Ja(\vtheta)$ as:
    \begin{align*}
        \Ja(\vtheta) = \E_{\underline{\vepsilon}} \left[\int_{\tau} p_{\mu_{\vtheta} + \underline{\vepsilon}}(\tau) \sum_{t=0}^{T-1} \gamma^t r(\vs_t, \mu_{\vtheta}(\vs_t)+ \vepsilon_t ) \right] = \E_{\underline{\vepsilon}} \left[\underbrace{\int_{\tau}  \sum_{t=0}^{T-1} p_{\mu_{\vtheta} + \underline{\vepsilon}}(\tau_{0:t}) \gamma^t r(\vs_t, \mu_{\vtheta}(\vs_t) + \vepsilon_t)}_{\eqqcolon f(\underline{\vepsilon})} \right],
    \end{align*}
    where $p_{\mu_{\vtheta} + \underline{\vepsilon}}(\tau)$ is the probability density function of the trajectory $\tau$ by acting via the deterministic policy $\mu_{\vtheta}$ perturbed by $\underline{\vepsilon}$, and $\tau_{0:t}$ is the trajectory $\tau$ considered from step $0$ to step $t$.
    Note that we call the term inside the expectation $f(\underline{\vepsilon})$.
    Moreover, $f(\bm{0})=\Jd(\vtheta)$.
    
    Using Taylor expansion, we have:
    \begin{align}
        \Ja(\vtheta) &= \E_{\underline{\vepsilon}}[f(\underline{\vepsilon})] \nonumber\\
        &= f(\bm{0}) +\E_{\underline{\vepsilon}}[ \underline{\vepsilon}^\top  \nabla_{\underline{\vepsilon}}  f(\underline{\vepsilon})\rvert_{\underline{\vepsilon} = \widetilde{\underline{\vepsilon}}}] \nonumber\\
        &=\Jd(\vtheta) + \sum_{t=0}^{T-1} \E_{\underline{\vepsilon}}[\vepsilon_t^\top \nabla_{\vepsilon_t} f(\underline{\vepsilon})\rvert_{\underline{\vepsilon} = \widetilde{\underline{\vepsilon}}}] \nonumber\\
        &\le \Jd(\vtheta) + \sum_{t=0}^{T-1} \E_{\underline{\vepsilon}}[\|\vepsilon_t\|_2^2]^{1/2}  \E_{\underline{\vepsilon}}[ \|\nabla_{\vepsilon_t} f(\underline{\vepsilon})\rvert_{\underline{\vepsilon} = \widetilde{\underline{\vepsilon}}}\|_2^2]^{1/2}. \label{pp:1}
    \end{align}
    
    We want to find a bound for the $ \|\nabla_{\vepsilon_t} f(\vepsilon)\rvert_{\underline{\vepsilon} = \widetilde{\underline{\vepsilon}}}\|_2^2$ which is different for every $t$, since we expect later time steps to be less relevant due to discounting. 
    We have for $k \in [0,T-1]$:
    \begin{align*}
        \left\| \nabla_{\underline{\vepsilon}_k} f(\underline{\vepsilon}) \right\|_2 
        &\leq \E_{\tau \sim p_{\mu_{\vtheta} + \underline{\vepsilon}}} \left[  \sum_{t=0}^{T-1} \left\| \nabla_{\underline{\vepsilon}_k} \log p_{\mu_{\vtheta} + \underline{\vepsilon}}(\tau_{0:t}) \right\|_2 \gamma^t |r(\vs_t, \mu_{\vtheta}(\vs_t)+ \underline{\vepsilon}_t )| +  \sum_{t=0}^{T-1} \gamma^t \|\nabla_{\underline{\vepsilon}_k} r(\vs_t, \mu_{\vtheta}(s_t)+ \underline{\vepsilon}_t )\|_2 \right] \\
        &  \leq \E_{\tau \sim p_{\mu_{\vtheta} + \underline{\vepsilon}}} \left[  \sum_{t=0}^{T-1}  \gamma^t |r(\vs_t, \mu_{\vtheta}(\vs_t)+ \underline{\vepsilon}_t ) |\sum_{l=0}^{t-1} \| \nabla_{\underline{\vepsilon}_k} \log p(\vs_{l+1}|\vs_l, \mu_{\vtheta}(s_l)+\underline{\vepsilon}_l)  \|_2  +  \sum_{t=0}^{T-1} \gamma^t \|\nabla_{\underline{\vepsilon}_k} r(\vs_t, \mu_{\vtheta}(\vs_t)+ \underline{\vepsilon}_t )\|_2 \right] \\
        &  = \E_{\tau \sim p_{\mu_{\vtheta} + \underline{\vepsilon}}} \left[  \sum_{t=k+1}^{T-1}  \gamma^t |r(\vs_t, \mu_{\vtheta}(\vs_t)+ \underline{\vepsilon}_t ) | \| \nabla_{\underline{\vepsilon}_k} \log p(\vs_{k+1}|\vs_k, \mu_{\vtheta}(\vs_k)+\underline{\vepsilon}_k)  \|_2  +  \gamma^k \|\nabla_{\underline{\vepsilon}_k} r(\vs_k, \mu_{\vtheta}(\vs_k)+ \underline{\vepsilon}_k )\|_2 \right] \\
        &\leq \sum_{t=k+1}^{T-1} \gamma^t  R_{\max}  L_{\log p} + \gamma^k L_r   \\
        & = \frac{\gamma^{k+1}-\gamma^T}{1-\gamma} L_{\log p}  R_{\max} + \gamma^k L_r .
    \end{align*}

    \todomp{Perchè la sommatoria su $l$ nella seconda riga è fino a $t-1$ e non fino a $t$? Perchè quella su $t$ nella terza riga parte da $k+1$ e non da $k$?}
    
    Thus, summing over $k$:
    \begin{align}
        \sum_{k=0}^{T-1} \E_{\underline{\vepsilon}}[ \|\nabla_{\underline{\vepsilon}_t} f(\underline{\vepsilon})\rvert_{\underline{\vepsilon} = \widetilde{\underline{\vepsilon}}}\|_2^2]^{1/2} &\le \sum_{t=0}^{T-1} \frac{\gamma^{k+1}-\gamma^T}{1-\gamma} L_{\log p}  R_{\max} + \gamma^k L_r \nonumber\\ 
        &= \frac{\gamma + \gamma^{1 + T} (T-1) - T \gamma^T }{(1-\gamma)^2} L_{\log p}  R_{\max} + \frac{1 - \gamma^T}{1 - \gamma} L_r. \label{pp:2}
    \end{align}

     Now, recalling that $ \E_{\underline{\vepsilon}}[\|\underline{\vepsilon}_t\|_2^2] \le \asigma^2 \da$, we have:

    % Given a $\vtheta \in \Theta$, we want to bound the quantity: $\left| \Jd(\vtheta) - \Ja(\vtheta) \right|$.

    \begin{align*}
        \left| \Jd(\vtheta) - \Ja(\vtheta) \right|
        &\leq \left| \sum_{t=0}^{T-1} \E_{\underline{\vepsilon}}[\|\vepsilon_t\|_2^2]^{1/2}  \E_{\underline{\vepsilon}}[ \|\nabla_{\vepsilon_t} f(\underline{\vepsilon})\rvert_{\underline{\vepsilon} = \widetilde{\underline{\vepsilon}}}\|_2^2]^{1/2} \right| \\
        &\leq\left| \sum_{t=0}^{T-1} \E_{\underline{\vepsilon}}[ \|\nabla_{\vepsilon_t} f(\underline{\vepsilon})\rvert_{\underline{\vepsilon} = \widetilde{\underline{\vepsilon}}}\|_2^2]^{1/2} \right| \asigma \sqrt{\da} \\
        &\leq \left( \frac{\gamma + \gamma^{1 + T} (T-1) - T \gamma^T }{(1-\gamma)^2} L_{\log p}  R_{\max} + \frac{1 - \gamma^T}{1 - \gamma} L_r \right) \asigma \sqrt{\da},
    \end{align*}
    where the first inequality is by Equation~\eqref{pp:1} and the last one is by Equation~\eqref{pp:2}.
\end{proof}

% As shown in the proof of Theorem~\ref{thr:assImpl}, 
    % %\todomp{broken ref}
    % the performance index $\Ja$ can be written as:
    % \begin{align*}
    %     \Ja(\vtheta) = \E_{\bvarepsilon} \left[\int_{\tau} p_{\mu_{\vtheta} + \bvarepsilon}(\tau) \sum_{t=0}^{T-1} \gamma^t r(\vs_t, \mu_{\vtheta}(\vs_t)+ \varepsilon_t ) \de\tau\right] = \E_{\bvarepsilon} \left[\int_{\tau}  \sum_{t=0}^{T-1} p_{\mu_{\vtheta} + \bvarepsilon}(\tau_{0:t}) \gamma^t r(\vs_t, \mu_{\vtheta}(\vs_t) + \varepsilon_t)\de\tau \right],
    % \end{align*}
    % where $\bvarepsilon = (\bvarepsilon_0, ..., \bvarepsilon_{T-1})^\top$ is a vector of $T$ noise vectors $\bvarepsilon_t$ sampled from $\mathcal{N}(\bm{0}_{\da}, \asigma^2 I_{\da})$.

    % In the following, we fix $\vtheta$ and abbreviate the term inside the expectation as $f(\bvarepsilon)$:
    % \begin{align*}
    %     f(\bvarepsilon) \coloneqq \int_{\tau}  \sum_{t=0}^{T-1} p_{\mu_{\vtheta} + \bvarepsilon}(\tau_{0:t}) \gamma^t r(\vs_t, \mu_{\vtheta}(\vs_t) + \varepsilon_t) \de\tau.
    % \end{align*}

    % Using Taylor expansion centered in $\bvarepsilon=\bm{0}$, noting $f({\bm 0})=J_D(\vtheta)$, we have:
    % \begin{align*}
    %     \Ja(\vtheta) &= \E_{\bvarepsilon}[f(\bvarepsilon)] \\
    %     &= f(\bm{0}) +\E_{\bvarepsilon}[ \bvarepsilon^\top  \nabla_{\bvarepsilon}  f(\bvarepsilon)\rvert_{\bvarepsilon = \widetilde{\bvarepsilon}}] \\
    %     &=f(\bm{0}) + \sum_{t=0}^{T-1} \E_{\bvarepsilon}[\varepsilon_t^\top \nabla_{\varepsilon_t} f(\bvarepsilon)\rvert_{\bvarepsilon = \widetilde{\bvarepsilon}}] \\
    %     &= \Jd(\vtheta) + \sum_{t=0}^{T-1} \E_{\bvarepsilon}[\varepsilon_t^\top \nabla_{\varepsilon_t} f(\bvarepsilon)\rvert_{\bvarepsilon = \widetilde{\bvarepsilon}}].
    % \end{align*}
    
	% We are interested in the gradient of $\Ja$:
 %    \begin{align*}
 %        \nabla_{\vtheta} \Ja(\vtheta) &= \nabla_{\vtheta} \Jd(\vtheta) + \sum_{t=0}^{T-1} \nabla_{\vtheta} \E_{\bvarepsilon}[\varepsilon_t^\top \nabla_{\varepsilon_t} f(\bvarepsilon)\rvert_{\bvarepsilon = \widetilde{\bvarepsilon}}] \\
 %        &= \nabla_{\vtheta} \Jd(\vtheta) + \sum_{t=0}^{T-1} \E_{\bvarepsilon}[\varepsilon_t^\top \nabla_{\vtheta} \nabla_{\varepsilon_t} f(\bvarepsilon)\rvert_{\bvarepsilon = \widetilde{\bvarepsilon}}].
 %    \end{align*}

    % Now, considering the norm of the gradient we have:
    % \begin{align*}
    %     \left\| \nabla_{\vtheta} \Ja(\vtheta)\right\|_2 &\geq \left\| \nabla_{\vtheta} \Jd(\vtheta) \right\|_2 - \left\| \sum_{t=0}^{T-1} \E_{\bvarepsilon}[\varepsilon_t^\top \nabla_{\vtheta} \nabla_{\varepsilon_t} f(\bvarepsilon)\rvert_{\bvarepsilon = \widetilde{\bvarepsilon}}] \right\|_2 \\
    %    &\geq \frac{1}{\dalpha} \left( \Jd^* - \Jd(\vtheta) \right) - \frac{\dbeta}{\dalpha} - \left\| \sum_{t=0}^{T-1} \E_{\bvarepsilon}[\varepsilon_t^\top \nabla_{\vtheta} \nabla_{\varepsilon_t} f(\bvarepsilon)\rvert_{\bvarepsilon = \widetilde{\bvarepsilon}}] \right\|_2 \\
    %     &\geq \frac{1}{\dalpha} \left( \Jd^* - \Jd(\vtheta) \right) - \frac{\dbeta}{\dalpha} - \sum_{t=0}^{T-1} \E_{\bvarepsilon}\left[\left\| \varepsilon_t^\top \right\|_2^2 \right]^{1/2} \E_{\bvarepsilon} \left[\left\| \nabla_{\vtheta} \nabla_{\varepsilon_t} f(\bvarepsilon)\rvert_{\bvarepsilon = \widetilde{\bvarepsilon}} \right\|_2^2 \right]^{1/2} \\
    %     &\geq \frac{1}{\dalpha} \left( \Jd^* - \Jd(\vtheta) \right) - \frac{\dbeta}{\dalpha} - \asigma \sqrt{\da} \sum_{t=0}^{T-1} \E_{\bvarepsilon} \left[\left\| \nabla_{\vtheta} \nabla_{\varepsilon_t} f(\bvarepsilon)\rvert_{\bvarepsilon = \widetilde{\bvarepsilon}} \right\|_2^2 \right]^{1/2},
    % \end{align*}    
    % where the second inequality is by Assumption~\ref{ass:Jd_gradient_domination}.
    
    % Re-arranging the last inequality, we have:
    % \begin{align*}
    %     \Jd^* - \Jd(\vtheta) \leq \dalpha \left\| \nabla_{\vtheta} \Ja(\vtheta)\right\|_2 + \dbeta + \dalpha \asigma \sqrt{\da} \sum_{t=0}^{T-1} \E_{\bvarepsilon} \left[\left\| \nabla_{\vtheta} \nabla_{\varepsilon_t} f(\bvarepsilon)\rvert_{\bvarepsilon = \widetilde{\bvarepsilon}} \right\|_2^2 \right]^{1/2}.
    % \end{align*}

    % In order to conclude the proof, we need to characterize the term $\sum_{t=0}^{T-1} \E_{\bvarepsilon} \left[\left\| \nabla_{\vtheta} \nabla_{\varepsilon_t} f(\bvarepsilon)\rvert_{\bvarepsilon = \widetilde{\bvarepsilon}} \right\|_2^2 \right]^{1/2}$.

    % From the proof of Theorem~\ref{thr:assImpl}, for any index $k \in \{0,\dots, T-1\}$, we have that:
    % \begin{align*}
    %     \nabla_{\bvarepsilon_{k}} f(\bvarepsilon) = \E_{\tau \sim p_{\mu_{\vtheta} + \bvarepsilon}} \left[ \sum_{t=k+1}^{T-1} \gamma^{t} r(s_{t}, \mu_{\vtheta}(s_{t}) + \bvarepsilon_{t}) \nabla_{\bvarepsilon_{k}} \log p(s_{k+1} | s_{k}, \mu_{\vtheta}(s_{k}) + \bvarepsilon_{k}) + \gamma^{k} \nabla_{\bvarepsilon_{k}} r(s_{k}, \mu_{\vtheta}(s_{k}) + \bvarepsilon_{k}) \right],
    % \end{align*}

    % from which we can derive $\nabla_{\vtheta} \nabla_{\bvarepsilon_{k}} f(\bvarepsilon)$ as follows:
    % \begin{align*}
    %     &\nabla_{\vtheta} \nabla_{\bvarepsilon_{k}} f(\bvarepsilon) \\
    %     &= \nabla_{\vtheta} \int_{\tau} p_{\mu_{\vtheta} + \bvarepsilon}(\tau) \left( \sum_{t=k+1}^{T-1} \gamma^{t} r(s_{t}, \mu_{\vtheta}(s_{t}) + \bvarepsilon_{t}) \nabla_{\bvarepsilon_{k}} \log p(s_{k+1} | s_{k}, \mu_{\vtheta}(s_{k}) + \bvarepsilon_{k}) + \gamma^{k} \nabla_{\bvarepsilon_{k}} r(s_{k}, \mu_{\vtheta}(s_{k}) + \bvarepsilon_{k}) \right) \\
    %     &= \int_{\tau} \nabla_{\vtheta} p_{\mu_{\vtheta} + \bvarepsilon}(\tau) \left( \sum_{t=k+1}^{T-1} \gamma^{t} r(s_{t}, \mu_{\vtheta}(s_{t}) + \bvarepsilon_{t}) \nabla_{\bvarepsilon_{k}} \log p(s_{k+1} | s_{k}, \mu_{\vtheta}(s_{k}) + \bvarepsilon_{k}) + \gamma^{k} \nabla_{\bvarepsilon_{k}} r(s_{k}, \mu_{\vtheta}(s_{k}) + \bvarepsilon_{k}) \right) \\
    %     &\qquad \qquad + p_{\mu_{\vtheta} + \bvarepsilon}(\tau) \nabla_{\vtheta} \left( \sum_{t=k+1}^{T-1} \gamma^{t} r(s_{t}, \mu_{\vtheta}(s_{t}) + \bvarepsilon_{t}) \nabla_{\bvarepsilon_{k}} \log p(s_{k+1} | s_{k}, \mu_{\vtheta}(s_{k}) + \bvarepsilon_{k}) + \gamma^{k} \nabla_{\bvarepsilon_{k}} r(s_{k}, \mu_{\vtheta}(s_{k}) + \bvarepsilon_{k}) \right) \\
    %     &= \E_{\tau \sim p_{\mu_{\vtheta} + \bvarepsilon}} \left[ \underbrace{\nabla_{\vtheta} \log p_{\mu_{\vtheta} + \bvarepsilon}(\tau) \left( \sum_{t=k+1}^{T-1} \gamma^{t} r(s_{t}, \mu_{\vtheta}(s_{t}) + \bvarepsilon_{t}) \nabla_{\bvarepsilon_{k}} \log p(s_{k+1} | s_{k}, \mu_{\vtheta}(s_{k}) + \bvarepsilon_{k}) + \gamma^{k} \nabla_{\bvarepsilon_{k}} r(s_{k}, \mu_{\vtheta}(s_{k}) + \bvarepsilon_{k}) \right)}_{\text{(i)}} \right.\\
    %     &\qquad \qquad \left. + \underbrace{\nabla_{\vtheta} \left( \sum_{t=k+1}^{T-1} \gamma^{t} r(s_{t}, \mu_{\vtheta}(s_{t}) + \bvarepsilon_{t}) \nabla_{\bvarepsilon_{k}} \log p(s_{k+1} | s_{k}, \mu_{\vtheta}(s_{k}) + \bvarepsilon_{k}) + \gamma^{k} \nabla_{\bvarepsilon_{k}} r(s_{k}, \mu_{\vtheta}(s_{k}) + \bvarepsilon_{k}) \right)}_{\text{(ii)}} \right].
    % \end{align*}

 %    We will consider the terms (i) and (ii) separately.

 %    However, we first need to clarify what happens when we try to compute the gradient \wrt $\vtheta$ and $\bvarepsilon_{t}$, for a generic $t \in \{0,\dots, T-1\}$.
 %    To this purpose let $g(\cdot, \va)$ be a generic differentiable function of the action $\va= \mu_{\vtheta}(s_t) + \bvarepsilon_t$.
	% The norm of its gradient \wrt $\bvarepsilon_t$ can be written as:
	% \begin{align*}
	% 	\| \nabla_{\bvarepsilon_t} g(\cdot, \va) \rvert_{\va = \mu_{\vtheta}(s_t) + \varepsilon_t} \|_2 &= \| \nabla_{\va}  g(\cdot, \va) \rvert_{\va = \mu_{\vtheta}(s_t) + \bvarepsilon_t} \nabla_{\bvarepsilon_t}(\mu_{\vtheta}(s_t) + \bvarepsilon_t) \|_2 \\
	% 	&= \|  \nabla_{\va}  g(\cdot, \va) \rvert_{\va = \mu_{\vtheta}(s_t) + \bvarepsilon_t} \|_2.
	% \end{align*}
	
	% On the other hand, the norm of the gradient of $g$ \wrt $\vtheta$ can be written as:
	% \begin{align*}
	% 		\| \nabla_{\vtheta} g(\cdot, \va) \rvert_{\va = \mu_{\vtheta}(s_t) + \bvarepsilon_t} \|_2 &= \| \nabla_{\va}  g(\cdot, \va) \rvert_{\va = \mu_{\vtheta}(s_t) + \bvarepsilon_t} \nabla_{\vtheta}(\mu_{\vtheta}(s_t) + \bvarepsilon_t) \|_2 \\
	% 		&= \| \nabla_{\va}  g(\cdot, \va) \rvert_{\va = \mu_{\vtheta}(s_t) + \bvarepsilon_t} \nabla_{\vtheta}\mu_{\vtheta}(s_t) \|_2.
	% \end{align*}
	
	% Moreover, the norm of the gradient \wrt $\vtheta$ of the gradient of $g$ \wrt $\bvarepsilon_t$, can be written as:
	% \begin{align*}
	% 		\| \nabla_{\vtheta} \nabla_{\bvarepsilon_t} g(\cdot, \va) \rvert_{\va = \mu_{\vtheta}(s_t) + \bvarepsilon_t} \|_2 &= \|  \nabla_{\vtheta} \nabla_{\va}  g(\cdot, \va) \rvert_{\va = \mu_{\vtheta}(s_t) + \bvarepsilon_t} \|_2 \\
	% 		&= \| \nabla_{\va}^2 g(\cdot, \va) \rvert_{\va = \mu_{\vtheta} + \bvarepsilon_t} \nabla_{\vtheta} \mu_{\vtheta}(s_t)\|_2.
	% \end{align*}
	
 %    Having said this, we can proceed by analyzing the terms (i) and (ii).

    % Term (i) can be written as:
    % \begin{align*}
    %     \text{(i)} &= \sum_{t=0}^{T-1} \nabla_{\vtheta} \log p(s_{t+1} | s_{t}, \mu_{\vtheta} + \bvarepsilon_{t}) \bigg( \sum_{t=k+1}^{T-1} \gamma^{t} r(s_{t}, \mu_{\vtheta}(s_{t}) + \bvarepsilon_{t}) \nabla_{\bvarepsilon_{k}} \log p(s_{k+1} | s_{k}, \mu_{\vtheta}(s_{k}) + \bvarepsilon_{k}) \\
    %     &\qquad \qquad + \gamma^{k} \nabla_{\bvarepsilon_{k}} r(s_{k}, \mu_{\vtheta}(s_{k}) + \bvarepsilon_{k}) \bigg).
    % \end{align*}

    % Thus, its norm can be bounded as:
    % \begin{align*}
    %     \left\| \text{(i)} \right\|_2 &\leq \sum_{t=0}^{T-1} \left\|\nabla_{\vtheta} \log p(s_{t+1} | s_{t}, \mu_{\vtheta} + \bvarepsilon_{t})\right\|_2 \bigg( \sum_{t=k+1}^{T-1} \gamma^{t} \left| r(s_{t}, \mu_{\vtheta}(s_{t}) + \bvarepsilon_{t}) \right| \left\|\nabla_{\bvarepsilon_{k}} \log p(s_{k+1} | s_{k}, \mu_{\vtheta}(s_{k}) + \bvarepsilon_{k})\right\|  \\
    %     &\qquad \qquad  + \gamma^{k} \left\| \nabla_{\bvarepsilon_{k}} r(s_{k}, \mu_{\vtheta}(s_{k}) + \bvarepsilon_{k})\right\|_2 \bigg) \\
    %     &\leq T L_{\log p} L_{\mu} \left( \frac{\gamma^{k+1} - \gamma^T}{1-\gamma} R_{\max} L_{\log p} + \gamma^k L_{r}\right).
    % \end{align*}
    % %\todomp{Qui c'è ancora il $T$}

    % Term (ii) can be written as:
    % \begin{align*}
    %     \text{(ii)} &= \sum_{t=k+1}^{T-1} \gamma^t \nabla_{\vtheta} r(s_{t}, \mu_{\vtheta}(s_{t}) + \bvarepsilon_{t}) \nabla_{\bvarepsilon_{k}} \log p(s_{k+1} | s_{k}, \mu_{\vtheta}(s_{k}) + \bvarepsilon_{k}) \\
    %     &\quad + \sum_{t=k+1}^{T-1} \gamma^t r(s_{t}, \mu_{\vtheta}(s_{t}) + \bvarepsilon_{t}) \nabla_{\vtheta} \nabla_{\bvarepsilon_{k}} \log p(s_{k+1} | s_{k}, \mu_{\vtheta}(s_{k}) + \bvarepsilon_{k}) \\
    %     &\quad + \gamma^k \nabla_{\vtheta} \nabla_{\bvarepsilon_{k}} r(s_{k}, \mu_{\vtheta}(s_{k}) + \bvarepsilon_{k}).
    % \end{align*}

    % Thus, its norm can be bounded as:
    % \begin{align*}
    %     \left\|\text{(ii)}\right\|_2 &\leq \sum_{t=k+1}^{T-1} \gamma^t \left\|\nabla_{\vtheta} r(s_{t}, \mu_{\vtheta}(s_{t}) + \bvarepsilon_{t})\right\|_2 \left\|\nabla_{\bvarepsilon_{k}} \log p(s_{k+1} | s_{k}, \mu_{\vtheta}(s_{k}) + \bvarepsilon_{k})\right\|_2 \\
    %     &\quad + \sum_{t=k+1}^{T-1} \gamma^t \left| r(s_{t}, \mu_{\vtheta}(s_{t}) + \bvarepsilon_{t}) \right| \left\|\nabla_{\vtheta} \nabla_{\bvarepsilon_{k}} \log p(s_{k+1} | s_{k}, \mu_{\vtheta}(s_{k}) + \bvarepsilon_{k})\right\|_2 \\
    %     &\quad + \gamma^k \left\| \nabla_{\vtheta} \nabla_{\bvarepsilon_{k}} r(s_{k}, \mu_{\vtheta}(s_{k}) + \bvarepsilon_{k}) \right\|_2 \\
    %     &\leq \frac{\gamma^{k+1} - \gamma^{T}}{1-\gamma} L_{\mu} \left( L_{r} L_{\log p} + R_{\max} L_{2 \log p} \right) + \gamma^k L_{2r} L_{\mu}.
    % \end{align*}

    % Putting together the bounds on $\text{(i)}$ and $\text{(ii)}$, we have that:
    % \begin{align*}
    %     \left\| \nabla_{\vtheta} \nabla_{\bvarepsilon_{k}} f(\bvarepsilon)\right\|_2 \leq T L_{\log p} L_{\mu} \left( \frac{\gamma^{k+1} - \gamma^T}{1-\gamma} R_{\max} L_{\log p} + \gamma^k L_{r}\right) + \frac{\gamma^{k+1} - \gamma^{T}}{1-\gamma} L_{\mu} \left( L_{r} L_{\log p} + R_{\max} L_{2 \log p} \right) + \gamma^k L_{2r} L_{\mu}.
    % \end{align*}

    % To conclude the proof, we just need to bound $\sum_{t=0}^{T-1} \E_{\bvarepsilon} \left[\left\| \nabla_{\vtheta} \nabla_{\varepsilon_t} f(\bvarepsilon)\rvert_{\bvarepsilon = \widetilde{\bvarepsilon}} \right\|_2^2 \right]^{1/2}$:
    % \begin{align*}
    %     \sum_{t=0}^{T-1} \E_{\bvarepsilon} \left[\left\| \nabla_{\vtheta} \nabla_{\varepsilon_t} f(\bvarepsilon)\rvert_{\bvarepsilon = \widetilde{\bvarepsilon}} \right\|_2^2 \right]^{1/2} 
    %     &\leq \sum_{t=0}^{T-1} T L_{\log p} L_{\mu} \left( \frac{\gamma^{t+1} - \gamma^T}{1-\gamma} R_{\max} L_{\log p} + \gamma^t L_{r}\right) \\&\qquad+ \sum_{t=0}^{T-1} \frac{\gamma^{t+1} - \gamma^{T}}{1-\gamma} L_{\mu} \left( L_{r} L_{\log p} + R_{\max} L_{2 \log p} \right) + \sum_{t=0}^{T-1} \gamma^t L_{2r} L_{\mu} \\
    %     &\leq \frac{\gamma (1-\gamma^T) - (1-\gamma)\gamma^T}{(1-\gamma)^2} L_{\mu} \left( R_{\max} T L_{\log p}^2 + L_{r} L_{\log p} + R_{\max} L_{2 \log p} \right) \\&\qquad+ \frac{1 - \gamma^T}{1 - \gamma} L_{\mu} \left( T L_{\log p} L_{r} + L_{2r}\right).
    % \end{align*}


The following theorem states the theoretical guarantees on the convergence to $\vtheta^*$ by running the generic algorithm $\mathfrak{A}$ under the previous assumptions.
Note that the derivation is a re-adaptation of the one presented by~\citet{yuan2022general} in their Theorem C.1.
\begin{thr} \label{thr:gen_conv}
	Under Assumptions~\ref{ass:J_wgd}, \ref{ass:J_gen_conv}, and \ref{ass:J_var_gen_conv}, given $\epsilon > 0$, we define $\delta$ such that: if $\epsilon' = 0$ then $\delta = \epsilon$, otherwise $\delta = \epsilon'$.
	Running the Algorithm $\mathfrak{A}$ for $K>0$ iterations with a batch size of $N$ trajectories tested in each iteration, and defining a learning rate $\zeta_k$ as:
	\begin{align*}
		\zeta_k =
		\begin{cases}
			\frac{1}{b} \quad &\text{if } K \leq \frac{b}{\mu \delta} \text{ or } k \leq k_0 \\
			\frac{4}{2b + \mu \delta (k - k_0)} \quad &\text{if } k > k_0
		\end{cases},
	\end{align*}
	where $b = \max\{\Lhgen; \  \mu \delta\}$, $\mu = \frac{1}{2 \alphagen^2}$, $\epsilon' = \frac{\betagen}{\alphagen}$ and $k_0 = \left[\frac{K}{2}\right]$.
	
	If $J^* - \E \left[J(\vtheta_{k})\right] \geq \delta \; \forall k \in \dsb{K}$, then
	\begin{align*}
		J^* - \E \left[J(\vtheta_{K})\right] \leq 16 \left(1 - \frac{\mu \delta}{2 b}\right)^{\left[\frac{K}{2}\right]} (J^* - J(\vtheta_{0})) + \frac{24 (2b - \Lhgen)}{\mu^2 \delta^2 K} (\epsilon')^2 + \frac{32 \Lhgen \Vgen}{N \mu^2 \delta^2 K} + \frac{4 \epsilon'}{\mu}.
	\end{align*}
	
	Otherwise, we have that:
	\begin{align*}
		\min_{k \in \dsb{K}} \left\{J^* - \E \left[J(\vtheta_{k})\right]\right\} \leq \delta.
	\end{align*}
\end{thr}
\begin{proof}
    Before starting the proof, we need a preliminary result that immediately follows from Assumption~\ref{ass:J_wgd}, by rearranging:
 %    , for which it holds that:
	% \begin{align*}
	% 	J(\vtheta^*) - J(\vtheta) \leq \alphagen \| \nabla_{\vtheta} J(\vtheta) \|_2 + \betagen.
	% \end{align*}
 
	\begin{align*}
		\frac{1}{\alphagen} \left(J(\vtheta^*) - J(\vtheta)\right) \leq \| \nabla_{\vtheta} J(\vtheta) \|_2 + \frac{\betagen}{\alphagen}.
	\end{align*}
 
	In the following, we use the notation $\epsilon' = \frac{\betagen}{\alphagen}$ and $\mu = \frac{1}{2 \alphagen^2}$.
	
	From such a result, we can write the following bound:
	\begin{align}
		\| \nabla_{\vtheta} J(\vtheta) \|_2^2 \geq 	\mu \left(J(\vtheta^*) - J(\vtheta)\right)^2 - (\epsilon')^2. \label{eq:duplicate_label}
	\end{align}
	
	Considering a $k \in \dsb{K}$ it follows that:
	\begin{align*}
		J(\vtheta^*) - J(\vtheta_{k+1}) 
        % &= J(\vtheta^*) - J(\vtheta_{k+1}) + J(\vtheta_{k}) - J(\vtheta_{k}) \\
		&=  J(\vtheta^*) - J(\vtheta_{k}) - ( J(\vtheta_{k+1}) - J(\vtheta_{k})) \\
		&\leq J(\vtheta^*) - J(\vtheta_{k}) - \left<  \vtheta_{k+1} - \vtheta_{k}; \nabla_{\vtheta}J(\vtheta_{k}) \right> + \frac{\Lhgen}{2} \|  \vtheta_{k+1} - \vtheta_{k} \|_2^2 \\
		&\leq J(\vtheta^*) - J(\vtheta_{k}) - \zeta_k \left< \widehat{\nabla}_{\vtheta}J(\vtheta_{k})  ; \nabla_{\vtheta}J(\vtheta_{k}) \right> + \frac{\Lhgen}{2} \zeta_k^2 \|  \widehat{\nabla}_{\vtheta}J(\vtheta_{k}) \|_2^2,
	\end{align*}

    where the second line follows by applying the Mean Value Theorem and exploiting Assumption~\ref{ass:J_gen_conv}, the last line, instead, follows from the fact that the parameter update is $\vtheta_{k+1} \leftarrow \vtheta_{k} + \zeta_k \widehat{\nabla}_{\vtheta} J(\vtheta_{k})$. 
	%\todomp{va spiegato perchè la prima inequality segue da Asm. B.2}

    In the following, we use the shorthand notation $\E_k[\cdot]$ to denote the conditional expectation w.r.t. the history up to the $k$-th iteration \emph{not} included. More formally, let $\mathcal{F}_k=\sigma\left(\vtheta_0,\mathcal{D}_0,\mathcal{D}_1,\dots,\mathcal{D}_k\right)$ be the $\sigma$-algebra encoding all the stochasticity up to iteration $k$ included. Note that all the stochasticity comes from the samples (except from the initial parameter $\vtheta_0$, which may be randomly initialized), and that $\vtheta_{k}$ is $\mathcal{F}_{k-1}$-measurable, that is, deterministically determined by the realization of the samples collected in the first $k-1$ iterations. Then, $\E_k[\cdot] \coloneqq \E[\cdot|\mathcal{F}_{k-1}]$. We will make use of the basic facts $\E[\cdot]=\E[\E_k[\cdot]]$ and $\E_k[X] = X$ for $\mathcal{F}_{k-1}$-measurable $X$. The variance of $\widehat{\nabla} J(\vtheta_k)$ must be always understood as conditional on $\mathcal{F}_{k-1}$.
  
	Now, 
    %we can consider the conditional expectation on $\vtheta_{k}$. 
    for any $k \in \dsb{K}$:
    \begin{align*}
		\E_k \left[ 	J(\vtheta^*) - J(\vtheta_{k+1}) \right] &\leq \E_k \left[ J(\vtheta^*) - J(\vtheta_{k}) - \zeta_k \left< \widehat{\nabla}_{\vtheta}J(\vtheta_{k})  ; \nabla_{\vtheta}J(\vtheta_{k}) \right> + \frac{\Lhgen}{2} \zeta_k^2 \|  \widehat{\nabla}_{\vtheta}J(\vtheta_{k}) \|_2^2 \right] \\
		&\leq J(\vtheta^*) - J(\vtheta_{k}) - \zeta_k \| \nabla_{\vtheta} J(\vtheta_{k}) \|_2^2+ \frac{\Lhgen}{2} \zeta_k^2 \E_k \left[\|  \widehat{\nabla}_{\vtheta}J(\vtheta_{k}) \|_2^2\right] \\
		&\leq J(\vtheta^*) - J(\vtheta_{k}) - \zeta_k \left(1 -  \frac{\Lhgen}{2} \zeta_k \right)  \| \nabla_{\vtheta} J(\vtheta_{k}) \|_2^2 + \frac{\Lhgen}{2} \zeta_k^2 \Var\left( \widehat{\nabla}_{\vtheta}J(\vtheta_{k}) \right) \\
		&\leq J(\vtheta^*) - J(\vtheta_{k}) - \zeta_k \left( 1 - \frac{\Lhgen}{2} \zeta_k \right)  \| \nabla_{\vtheta} J(\vtheta_{k}) \|_2^2 + \frac{\Lhgen \Vgen}{2N} \zeta_k^2,
	\end{align*}

	where the third inequality follows from the fact that $\widehat{\nabla}_{\vtheta} J(\vtheta)$ is an unbiased estimator, and from the definition of $\Var(\widehat{\nabla} J(\vtheta))$.
	
	Now, selecting a step size $\zeta_k \leq \frac{1}{\Lhgen}$, we can use the bound from Equation~(\ref{eq:genconv_eq_1}):
	\begin{align*}
			\E_k &\left[ J(\vtheta^*) - J(\vtheta_{k+1}) \right] \\
			&\leq J(\vtheta^*) - J(\vtheta_{k}) - \zeta_k \left( 1 - \frac{\Lhgen}{2} \zeta_k \right) \left( \mu \left(J(\vtheta^*) - J(\vtheta_{k})\right)^2 - (\epsilon')^2 \right) + \frac{\Lhgen \Vgen}{2N} \zeta_k^2 \\
			&\leq J(\vtheta^*) - J(\vtheta_{k}) - \mu \zeta_k \left( 1 - \frac{\Lhgen}{2} \zeta_k \right) \left( J(\vtheta^*) - J(\vtheta_{k}) \right)^2 +  \zeta_k \left( 1 - \frac{\Lhgen}{2} \zeta_k \right) (\epsilon')^2 + \frac{\Lhgen \Vgen}{2N} \zeta_k^2.
	\end{align*}

	The next step is to consider the total expectation over both the terms of the inequality.
	In particular, we define $r_k \coloneqq \E \left[J(\vtheta^*) - J(\vtheta_{k})\right]$.
    \todomp{leggendo la proof di Alberto mi sono accorto di un possibile errore (ereditato da Yuan). Mi sa che bisogna definire $r_k=\E_{k-1}[J(\vtheta^*)-J(\vtheta_{k})]$ con la conditional e fare la total expectation alla fine...perchè definendo $r_k$ con la total expectation non è mica vero che quello qui sotto è $r_k^2$. Con la conditional mi sembra che funzioni visto che alla fine della ricorsione restano solo $r_K$ e $r_0$ a cui si può applicare total expectation}
    \am{E' vero. Non ci avevo fatto caso...}
	We can then rewrite the previous inequality as follows:
	\begin{align*}
		r_{k+1} \leq r_k - \mu \zeta_k \left( 1 - \frac{\Lhgen}{2} \zeta_k \right) r_k^2 +  \zeta_k \left( 1 - \frac{\Lhgen}{2} \zeta_k \right) (\epsilon')^2 + \frac{\Lhgen \Vgen}{2N} \zeta_k^2.
	\end{align*}

	If $\exists \overbar{k} \in \dsb{K}$ such that $r_{\overbar{k}} < \delta$, we are done.
    Indeed, in this case we found an iteration index $\overbar{k}$ such that $\E\left[ J^* - J(\vtheta_{\overbar{k}}) \right] \leq \delta$.
    %\todomp{perchè?}
	Otherwise, if $r_k \geq \delta$ for all $k \in \dsb{K}$, we can proceed as follows:
	\begin{align}
			r_{k+1} &\leq r_k - \mu \zeta_k \delta \left( 1 - \frac{\Lhgen}{2} \zeta_k \right) r_k +  \zeta_k \left( 1 - \frac{\Lhgen}{2} \zeta_k \right) (\epsilon')^2 + \frac{\Lhgen \Vgen}{2N} \zeta_k^2 \nonumber \\
			&\leq \left( 1 - \mu \zeta_k \delta \left( 1 - \frac{\Lhgen}{2} \zeta_k \right)  \right) r_k +  \zeta_k \left( 1 - \frac{\Lhgen}{2} \zeta_k \right) (\epsilon')^2 + \frac{\Lhgen \Vgen}{2N} \zeta_k^2 \nonumber \\
			&\leq  \left( 1 - \frac{\mu \delta \zeta_k}{2}  \right) r_k +  \zeta_k \left( 1 - \frac{\Lhgen}{2} \zeta_k \right) (\epsilon')^2 + \frac{\Lhgen \Vgen}{2N} \zeta_k^2, \label{eq:genconv_eq_2}
	\end{align}
	where the last line follows from our choice of step size $\zeta_k \leq \frac{1}{\Lhgen}$.
	
	For what follows, it is worth noting that $1 - \mu \delta \zeta_k \geq 0$ for $\zeta_k \leq \frac{1}{b}$ with $b \geq \mu \delta$, so we need to consider two different cases.
 
    \textbf{Case 1:} $K \leq \frac{b}{\mu \delta}$. We set $\zeta_k = \frac{1}{b}$, and thus we can derive what follows:
	\begin{align}
		r_K &\leq \left( 1 - \frac{\mu \delta}{2b} \right) r_{K-1} + \frac{2b - \Lhgen}{2 b^2} (\epsilon')^2 + \frac{\Lhgen \Vgen}{2 N b^2} \nonumber\\
		&\leq \left( 1 - \frac{\mu \delta}{2b} \right)^K r_{0} + \left(  \frac{2b - \Lhgen}{2 b^2} (\epsilon')^2 + \frac{\Lhgen \Vgen}{2 N b^2} \right) \sum_{i=0}^{K-1} \left(1 - \frac{\mu \delta}{2b}\right)^i \nonumber\\
		&\leq  \left( 1 - \frac{\mu \delta}{2b} \right)^K r_0 +  \frac{2b - \Lhgen}{\mu \delta b} (\epsilon')^2 + \frac{\Lhgen \Vgen}{N \mu \delta b} \nonumber\\
		&\leq  \left( 1 - \frac{\mu \delta}{2b} \right)^K r_0 +  \frac{2b - \Lhgen}{\mu^2 \delta^2 K} (\epsilon')^2 + \frac{\Lhgen \Vgen}{N \mu^2 \delta^2 K}. \label{eq:genconv_eq_3}
	\end{align}
	
	\textbf{Case 2:} $K \geq \frac{b}{\mu \delta}$. In such a case, it does not suffice to unroll the recursion of line~(\ref{eq:genconv_eq_2}) and then apply a bound on the $K$ to highlight the dependence on the number of iterations itself.
	Instead, it is useful to define the quantity:
	\begin{align*}
		k_0 \coloneqq \left\lceil\frac{K}{2}\right\rceil \geq \frac{K-1}{2}.
	\end{align*}
 
	Now we can think of two cases: the one in which $k \leq k_0$ and the one in which $k > k_0$.

	When $k \leq k_0$, we can resume from line~(\ref{eq:genconv_eq_2}) and perform a similar argument as in Case 1. 
    % the case in which $K \leq \frac{b}{\mu \delta}$. 
	This gives us a bound on the quantity $r_{k_0}$ which will be useful later on.
	Setting $\zeta_k = \frac{1}{b}$ with $b \geq \mu \delta$, we can easily obtain:
	\begin{align}
		r_{k_0} &\leq \left(1 - \frac{\mu \delta}{2 b}\right)^{k_0} r_0 + \frac{2b - \Lhgen}{\mu \delta b} (\epsilon')^2 + \frac{\Lhgen \Vgen}{N \mu \delta b} \nonumber \\
		&=\left(1 - \frac{\mu \delta}{2 b}\right)^{\left\lceil \frac{K}{2} \right\rceil} r_0 + \frac{2b - \Lhgen}{\mu \delta b} (\epsilon')^2 + \frac{\Lhgen \Vgen}{N \mu \delta b}.  \label{eq:genconv_eq_4}
	\end{align}
	
	When $k > k_0$, we need to select an adaptive learning rate as:
	\begin{align*}
		\zeta_k = \frac{4}{\mu \delta \left(\frac{2b}{\mu \delta} + k - k_0\right)}.
	\end{align*}
	
	Now, we can resume from line~(\ref{eq:genconv_eq_2}) as follows:
	\begin{align*}
		r_{k} &\leq \left(1 - \frac{\mu \delta \zeta_k}{2}\right) r_{k-1} + \zeta_k \left( 1 - \frac{\Lhgen}{2} \zeta_k \right) (\epsilon')^2 + \frac{\Lhgen \Vgen}{2N} \zeta_k^2 \\
		&\leq \frac{\frac{2b}{\mu \delta} + k - k_0 - 2 }{\frac{2b}{\mu \delta} + k - k_0} r_{k-1} + \frac{4 \mu \delta \left(\frac{2b}{\mu \delta} + k - k_0 \right) - 8 \Lhgen}{\mu^2 \delta^2 \left( \frac{2b}{\mu \delta} +k - k_{0} \right)^{2}} (\epsilon')^2 + \frac{8 \Lhgen \Vgen}{N \mu^2 \delta^2 \left(\frac{2b}{\mu \delta} + k - k_0 \right)^2}. 
	\end{align*}
    %\ale{da qui fixare 8}
	We now need to define $w_k \coloneqq \left(\frac{2b}{\mu \delta} + k - k_0 \right)^2$.
	Then, multiplying both sides of the inequality by $w_k$, we obtain:
	\begin{align*}
		w_k r_k &\leq \left(\frac{2b}{\mu \delta} + k - k_0 \right) \left(\frac{2b}{\mu \delta} + k - k_0 - 2\right) r_{k-1} + 	\frac{4}{\mu \delta} \left(\frac{2b - 2 \Lhgen}{\mu \delta} + k - k_0 \right) (\epsilon')^2 + \frac{8\Lhgen \Vgen}{N \mu^2 \delta^2} \\
		&= \left(\frac{2b}{\mu \delta} + k - k_0 - 1 \right)^2 r_{k-1} + \frac{4}{\mu \delta} \left(\frac{2b - 2 \Lhgen}{\mu 	\delta} + k - k_0 \right) (\epsilon')^2 + \frac{8\Lhgen \Vgen}{N \mu^2 \delta^2} \\
		&= w_{k-1} r_{k-1} + \frac{4}{\mu \delta} \left(\frac{2b - 2 \Lhgen}{\mu \delta} + k - k_0 \right) (\epsilon')^2 + 	\frac{8\Lhgen \Vgen}{N \mu^2 \delta^2}.
	\end{align*}
	
	We can telescope from $k_0 + 1$ to $K$ the terms on both sides of the last inequality, obtaining
	\begin{align*}
		w_K r_K &\leq w_{k_0} r_{k_0} + \frac{4}{\mu \delta} (\epsilon')^2 \sum_{i=k_0+1}^{K} \left( \frac{2b - 2 \Lhgen}{\mu \delta} + k - k_0 \right) + \frac{8\Lhgen \Vgen}{N \mu^2 \delta^2} (K - k_0) \\
		&= \frac{4b^2}{\mu^2 \delta^2} r_{k_0} + \frac{4 (2b - 2 \Lhgen)}{\mu^2 \delta^2} (K - k_0) (\epsilon')^2 + \frac{2 (\epsilon')^2}{\mu \delta} (K - k_0) (K - k_0 + 1) + \frac{8\Lhgen \Vgen}{N \mu^2 \delta^2} (K - k_0).
	\end{align*}
	
	To continue the derivation, we divide both sides of the inequality by $w_K$. 
	Moreover, we use the fact that $w_K \geq (K - k_0)^2$ and the fact that $K - k_0 \geq \frac{K}{2}$.
	Thus, we can write:
	\begin{align*}
		 r_K &\leq  \frac{4b^2}{\mu^2 \delta^2 w_K} r_{k_0} + \frac{4 (2b - 2 \Lhgen)}{\mu^2 \delta^2 w_K} (K - k_0) (\epsilon')^2 + \frac{2 (\epsilon')^2}{\mu \delta w_K} (K - k_0) (K - k_0 + 1) + \frac{8\Lhgen \Vgen}{N \mu^2 \delta^2 w_K} (K - k_0) \\
		 &\leq \frac{16b^2}{\mu^2 \delta^2 K^2} r_{k_0} + \frac{4 (2b - 2 \Lhgen)}{\mu^2 \delta^2 (K- k_0)} (\epsilon')^2 + \frac{4 (\epsilon')^2}{\mu \delta} + \frac{8\Lhgen \Vgen}{N \mu^2 \delta^2 (K-k_0)} \\
		 &\leq \frac{16b^2}{\mu^2 \delta^2 K^2} r_{k_0} + \frac{8 (2b - 2 \Lhgen)}{\mu^2 \delta^2 K} (\epsilon')^2 + \frac{4 \epsilon'}{\mu} + \frac{16\Lhgen \Vgen}{N \mu^2 \delta^2 K},
	\end{align*}
    %\todomp{nella seconda inequality hai usato $(K-k_0+1)\le2(K-k_0)$ per il terzo termine? }
	where the last step is possible due to the fact that $\frac{(\epsilon')^2}{\delta} = \epsilon'$, recalling that $\epsilon'$ is either zero or equal to $\delta$.
	
	Finally, by employing the bound for $r_{k_0}$ obtained in Equation~(\ref{eq:genconv_eq_4}) we can conclude the analysis of Case 2 as:
	\begin{align}
		r_K &\leq \frac{16b^2}{\mu^2 \delta^2 K^2} \left( \left(1 - \frac{\mu \delta}{2 b}\right)^{\left[\frac{K}{2}\right]} r_0 + \frac{2b - \Lhgen}{\mu \delta b} (\epsilon')^2 + \frac{\Lhgen \Vgen}{N \mu \delta b} \right) + \frac{8 (2b - 2 \Lhgen)}{\mu^2 \delta^2 K} (\epsilon')^2 + \frac{4 \epsilon'}{\mu} + \frac{16\Lhgen \Vgen}{N \mu^2 \delta^2 K} \nonumber \\
		&\leq 16  \left(1 - \frac{\mu \delta}{2 b}\right)^{\left[\frac{K}{2}\right]} r_0 + \frac{24 (2b - \Lhgen)}{\mu^2 \delta^2 K} (\epsilon')^2 + \frac{32 \Lhgen \Vgen}{N \mu^2 \delta^2 K} + \frac{4 \epsilon'}{\mu}, \label{eq:gen_conv_eq_5}
	\end{align}
	where we used the fact that $K \geq \frac{b}{\mu \delta}$ in the case under examination.

    Finally, having studied the two cases, we need to consider the maximum bound between the one shown in Equation~(\ref{eq:genconv_eq_3}) and the one shown in Equation~(\ref{eq:gen_conv_eq_5}).
    \begin{align*}
        J(\vtheta^*) - \E\left[J(\vtheta_{K})\right] \leq 16  \left(1 - \frac{\mu \delta}{2 b}\right)^{\left[\frac{K}{2}\right]} \left( J(\vtheta^*) - J(\vtheta_{0}) \right) + \frac{24 (2b - \Lhgen)}{\mu^2 \delta^2 K} (\epsilon')^2 + \frac{32 \Lhgen \Vgen}{N \mu^2 \delta^2 K} + \frac{4 \epsilon'}{\mu}.
    \end{align*}
\end{proof}

==> contents/04_convergence.tex <==
In this section, we present our main results about the convergence of AB and PB \emph{white noise-based exploration} to  \emph{global optimal parameter} $\vtheta^*_{\text{D}}$ of the performance of the deterministic policy $\Jd$.
%algorithms GPODMP~\citep{baxter2001infinite} and PGPE~\citep{SEHNKE2010551} employing (hyper)policies complying with Definition~\ref{defi:add}.
Let $K \in \mathbb{N}$ be the number of \emph{iterations} and $N$ the \emph{batch size}; 
%(trajectories for AB exploration and parameter-trajectory pairs for PB exploration collected at each iteration). 
given an accuracy threshold $\epsilon > 0$, our goal is to bound the \emph{sample complexity} $NK$ to fulfill the following  \emph{last-iterate global} convergence condition:
\begin{align}\label{eq:conver}
   \Jd^* - \E \left[ \Jd(\vtheta_{K}) \right] \leq \epsilon,
\end{align}
where $\vtheta_{K}$ is the (hyper)parameter at the end of learning.
%To ensure convergence to the global optimum, we will make use of the \emph{Weak Gradient Domination} (WGD) property that is the gold standard for the global convergence of stochastic optimization algorithms~\cite{yuan2022general,masiha2022stochastic,fatkhullin2023stochastic}.
We start in Section~\ref{sec:generalConv}, introducing the \emph{abstract} assumptions and providing a general convergence analysis applicable to both AB and PB exploration for learning the corresponding objective ($\Ja$ or $\Jp$). Then, in Sections~\ref{sec:globalPGPE} and \ref{sec:globalPG}, we derive the convergence guarantees on the deterministic objective $\Jd$ for AB and PB exploration, respectively. Our results are first presented for a \emph{fixed} white noise variance $\sigma$ to highlight the trade-off between sample complexity and performance, then, extended to an \emph{$\epsilon$-adaptive} choice of $\sigma$.

\subsection{General Convergence Analysis}\label{sec:generalConv}
In this section, we provide a global convergence analysis for a generic stochastic first-order algorithm optimizing the differentiable objective function $J_\simbolo$ on the parameters space $\Theta \subseteq \mathbb{R}^d$, that can be instanced for AB (setting $J_\simbolo=\Ja$) and PB (setting $J_\simbolo=\Jp$) exploration. At every iteration $k \in \dsb{K}$, the algorithm performs the gradient ascent update:
\begin{align}\label{eq:update}
     \vtheta_{k + 1} \xleftarrow{} \vtheta_{k} + \zeta_{k} \widehat{\nabla}_{\vtheta} J_\simbolo(\vtheta_k),
\end{align}
where $\zeta_k>0$ is the \emph{step size} and $\widehat{\nabla}_{\vtheta} J_\simbolo(\vtheta_{k})$ is an \emph{unbiased} estimate of $\nabla_{\vtheta} J_\simbolo(\vtheta_{k})$. We denote $J^*_\simbolo = \max_{\vtheta \in \Theta} J_\simbolo(\vtheta)$. We enforce the following standard assumptions.

\begin{ass}[\sethlcolor{vibrantTeal!30}\hl{Weak gradient domination for $J_\simbolo$}] \label{ass:J_wgd}
    There exist $\alphagen > 0$ and $\betagen \geq 0$ such that  for every $ \vtheta \in \Theta$ it holds that $J^*_\simbolo - J_\simbolo(\vtheta) \leq \alphagen \|\nabla_{\vtheta} J_\simbolo (\vtheta) \|_2 + \betagen$.
\end{ass}

Assumption~\ref{ass:J_wgd} is the gold standard for the global convergence of stochastic optimization~\citep{yuan2022general,masiha2022stochastic,fatkhullin2023stochastic}. Note that, when $\beta = 0$, then we recover the (strong) \emph{gradient domination} (GD) property: $J^*_\simbolo - J_\simbolo(\vtheta) \leq \alpha \left\| \nabla_{\vtheta} J(_\simbolo\vtheta) \right\|_2$ for all $\vtheta\in\Theta$.
GD is stricter than WGD, and requires that $J_\simbolo$ has no local optima. Instead, WGD admits local maxima as long as their performance is $\beta$-close to the globally optimal one.\footnote{In this section, we will assume that $J_\simbolo$ (i.e., either $\Ja$ or $\Jd$) is already endowed with the WGD property. In Section~\ref{sec:assumptions}, we illustrate how it can be obtained in several common scenarios.} %We remark that the WGD property can be assumed directly on the objectives $\Ja$ and $\Jp$ or inherited from the deterministic objective $$ as shown in Section~\ref{}.

\begin{ass}[\sethlcolor{vibrantMagenta!30}\hl{Smooth $J_\simbolo$ w.r.t. parameters $\vtheta$}]\label{ass:J_gen_conv}
    $J$ is $L_{2,\simbolo}$-LS \wrt parameters $\vtheta$, \ie for every $\vtheta,\vtheta' \in \Theta$, it holds that:
    \begin{align}
        \|\nabla_{\vtheta} J_\simbolo(\vtheta') - \nabla_{\vtheta} J_\simbolo(\vtheta)\|_2 \le L_{2,\simbolo} \| \vtheta' - \vtheta \|_2.
    \end{align}
    % \begin{itemize}[noitemsep]
    %     \item $\exists \Lgen \geq 0$ such that $\forall \vtheta, \vtheta' \in \Theta$ it holds that $|J(\vtheta) - J(\vtheta')| \leq \Lgen \| \vtheta - \vtheta'\|_2$
    %     \am{La usi questa prima assunzione nella proof?}
    %     \item $\exists \Lhgen \geq 0$ such that $\forall \vtheta \in \Theta$ it holds that $\| \nabla_{\vtheta}^2 J(\vtheta) \|_2 \leq \Lhgen$
    % \end{itemize}
\end{ass}

Assumption~\ref{ass:J_gen_conv} is ubiquitous in the convergence analysis of policy gradient algorithms~\cite{papini2018stochastic, bhandari2019global, agarwal2021theory,yuan2022general}, it is usually studied as an instance of (non-convex) \emph{smooth} stochastic optimization. 
%{\color{blue}It is often stated in the equivalent (for twice differentiable $J$) form $\norm[2][]{\nabla_{\vtheta}^2J_\simbolo(\vtheta)}\le L_{2,\simbolo}$, as an upper bound on the spectral norm of the Hessian.} 
As shown in Table~\ref{tab:magic}, the smoothness of $J_\simbolo \in \{\Ja,\Jp\}$ can be: ($i$) inherited from the deterministic objective $\Jd$ (originating, in turn, from the regularity of the MDP) and of the deterministic policy $\bm{\mu}_{\vtheta}$ (Asm.~\ref{ass:lipMdp}-\ref{ass:smoothPol}); or ($ii$) enforced through the properties on the white noise $\Phi$ (Asm.~\ref{ass:magic}). {The first result was observed in a similar form by~\citet[][Theorem 3]{pirotta2015policy}, while a generalization of the second was established by~\citet{papini2022smoothing} and refined by~\citet{yuan2022general}.}

\begin{ass}[\sethlcolor{vibrantBlue!30}\hl{Bounded estimator variance $\widehat{\nabla}_{\vtheta} J_\simbolo(\vtheta)$}]\label{ass:J_var_gen_conv}
    The estimator $\widehat{\nabla}_{\vtheta} J_\simbolo(\vtheta)$ computed with batch size $N$ has a bounded variance, i.e., there exists $ \Vgen \geq 0$ such that, for every $ \vtheta \in \Theta$, we have:  $\Var[\widehat{\nabla}_{\vtheta} J_\simbolo(\vtheta)] \leq V_\simbolo/N$.
\end{ass}

Assumption~\ref{ass:J_var_gen_conv} guarantees that the gradient estimator is characterized by a bounded variance $V_\simbolo$ which scales with the batch size $N$. Under Assumptions~\ref{ass:magic} (and~\ref{ass:smoothMdp}-\ref{ass:smoothPol}), the term $V_\simbolo$ can be further characterized as in Table~\ref{tab:magic}.

We are now ready to state the global convergence result.

\begin{restatable}{thr}{globalConvGeneral}\label{thr:gen_conv_new}
    Consider an algorithm running the update rule of Equation~\eqref{eq:update}. Under Assumptions~\ref{ass:J_wgd}, \ref{ass:J_gen_conv}, and~\ref{ass:J_var_gen_conv}, with a suitable constant step size, to guarantee $
         J_\simbolo^* - \E[J_\simbolo(\vtheta_K)] \le \epsilon + \beta
$ the sample complexity is at most:
     \begin{align}
         NK =  \frac{16\alpha^4L_{2,\simbolo}V_\simbolo}{\epsilon^3} \log \frac{\max\{0,J^*_\simbolo - J_\simbolo(\vtheta_0) - \beta\}}{\epsilon}.
 \end{align}
\end{restatable}

This result establishes a convergence of order $\widetilde{O}(\epsilon^{-3})$ to the global optimum $J^*_\simbolo$ of the general objective $J_\simbolo$. Recalling that $J_\simbolo \in \{\Ja,\Jp\}$, Theorem~\ref{thr:gen_conv_new} provides: ($i$) the first global convergence guarantee for PGPE for PB exploration(setting $J_\simbolo=\Jp$) and ($ii$) a global convergence guarantee for PG for AB exploration of the same order (up to logarithmic terms in $\epsilon^{-1}$) of the state-of-the-art one of~\citet{yuan2022general} (setting $J_\simbolo=\Ja$). Note that our guarantee is obtained for a \emph{constant} step size and holds for the last parameter $\vtheta_K$, delivering a \emph{last-iterate} result, rather than a \emph{best-iterate} one as in~\citep[][Corollary 3.7]{yuan2022general}. Clearly, this result is not yet our ultimate goal since, we need to assess how far the performance of the learned parameter $\vtheta_K$ is from that of the optimal deterministic objective $\Jd^*$.

% \begin{table*}[t]
%     \centering\renewcommand{\arraystretch}{1.2}
%     \resizebox{\linewidth}{!}{\begin{tabular}{|C{2.5cm}|C{2.5cm}|C{6.5cm}|C{3cm}|C{3cm}|}\hline
%          &  $L_{\star} $ (Lipschitz) & \multicolumn{2}{c|}{ $L_{2,\star}$ (Smooth)} &   $V_{\star}$ (Variance bound)\\ \hline
%          \textbf{\textcolor{vibrantBlue}{AB Exploration}}  ($\star$=A)& \cellcolor{brightYellow!30} $  \frac{L_p R_{\max}}{(1-\gamma)^2} + \frac{ L_r}{1 - \gamma} $ &  \cellcolor{vibrantMagenta!30} $ \frac{L_p^2 L_\mu^2 R_{\max}}{(1-\gamma)^3} + \frac{2L_\mu^2L_p L_r+ L_{2,\mu}L_{2,p}R_{\max} }{(1-\gamma)^2} + \frac{L_{2,\mu}L_{2,r}}{1-\gamma}  $  &  \cellcolor{vibrantMagenta!30}  $ \frac{R_{\max}c (\da+1)(L_\mu^2 + L_{2,\mu})}{\sigma^2_\text{A}(1-\gamma)^2} $ & \cellcolor{vibrantBlue!30}  $ \frac{R_{\max} c \da L_\mu^2}{\sigma_{\text{A}}^2(1-\gamma)^3}$ \\\cdashline{2-5}
%          {\small \hfill  Assumptions:} & {\small \ref{ass:lipMdp}} & {\small \ref{ass:lipMdp}, \ref{ass:lipPol}, \ref{ass:smoothMdp}, \ref{ass:smoothPol} } & {\small  \ref{ass:lipPol}, \ref{ass:smoothPol}, \ref{ass:magic}} & {\small \ref{ass:magic}, \ref{ass:lipPol} } \\\cdashline{2-5}
%          {\small \hfill Reference:}  & {\small Lemma~\ref{thr:assImpl}} 
%          &  \multicolumn{2}{c|}{\small Lemma~\ref{lem:Ja_bounded_hessian}^{$\ddagger$}}&  {\small Lemma \ref{ass:Ja_estim_bounded_variance}} \\\hline
%          \textbf{\textcolor{vibrantRed}{PB Exploration}}  ($\star$=P)& $ \cellcolor{brightYellow!30}  \frac{L_p L_\mu R_{\max}}{(1-\gamma)^2} + \frac{ L_r L_\mu }{1 - \gamma} $  & \cellcolor{vibrantMagenta!30} $ \frac{L_p^2 L_\mu^2 R_{\max}}{(1-\gamma)^3} + \frac{2L_\mu^2L_p L_r+ L_{2,\mu}L_{2,p}R_{\max} }{(1-\gamma)^2} + \frac{L_{2,\mu}L_{2,r}}{1-\gamma}  $ & \cellcolor{vibrantMagenta!30} $ \frac{R_{\max}c (\dt+1)}{\sigma^2_\text{P}(1-\gamma)^2} $  & \cellcolor{vibrantBlue!30} $  \frac{R_{\max} c \dt}{\sigma_{\text{P}}^2(1-\gamma)^2}$ \\\cdashline{2-5}
%          {\small \hfill Assumptions:} & {\small \ref{ass:lipMdp}, \ref{ass:lipPol} } & {\small \ref{ass:lipMdp}, \ref{ass:lipPol}, \ref{ass:smoothMdp}, \ref{ass:smoothPol} } & {\small \ref{ass:magic}} & {\small \ref{ass:magic} } \\\cdashline{2-5}
%          {\small \hfill Reference:}  & {\small Lemma~\ref{thr:assImpl}} 
%          &   \multicolumn{2}{c|}{\small Lemma~\ref{lem:Jp_bounded_hessian}}  &  {\small Lemma~\ref{ass:Jp_estim_bounded_variance}} \\
%          \hline
%     \end{tabular}}%
%     \caption{Caption. ${}^\ddagger$ for $\sigma_{\text{A}} < \sqrt{\da}$.}\label{tab:magic}
% \end{table*}

\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\begin{table*}[t]
    \centering
    \renewcommand{\arraystretch}{1}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{|C{2.5cm}|C{2.8cm}|C{6.7cm}|C{3.2cm}|C{3cm}|}\hline
             & $L_{\dagger} $ (Lipschitz) & \multicolumn{2}{c|}{ $L_{2,\dagger}$ (Smooth)} &   $V_{\dagger}$ (Variance bound)\\ \hline
             \textbf{\textcolor{vibrantBlue}{AB Exploration}}  ($\dagger$=A) & \cellcolor{brightYellow!30} $  \frac{L_p R_{\max}}{(1-\gamma)^2} + \frac{ L_r}{1 - \gamma} $ & \cellcolor{vibrantMagenta!30} $ \frac{2L_p^2 L_\mu^2 R_{\max}}{(1-\gamma)^3} + \frac{2L_\mu^2L_p L_r+ L_{2,\mu}L_{2,p}R_{\max} }{(1-\gamma)^2} + \frac{L_{2,\mu}L_{2,r}}{1-\gamma}  $  & \cellcolor{vibrantMagenta!30}  $ \frac{R_{\max}c (\da+1)(L_\mu^2 + L_{2,\mu})}{\sigma^2_\text{A}(1-\gamma)^2} $\textsuperscript{$\ddagger$} & \cellcolor{vibrantBlue!30}  $ \frac{R_{\max} c \da L_\mu^2}{\sigma_{\text{A}}^2(1-\gamma)^3}$ \\\cdashline{2-5}
             {\small \hfill  Assumptions:} & {\small \ref{ass:lipMdp}} & {\small \ref{ass:lipMdp}, \ref{ass:lipPol}, \ref{ass:smoothMdp}, \ref{ass:smoothPol} } & {\small  \ref{ass:lipPol}, \ref{ass:smoothPol}, \ref{ass:magic}} & {\small \ref{ass:magic}, \ref{ass:lipPol} } \\\cdashline{2-5}
             {\small \hfill Reference:}  & {\small Lemma~\ref{thr:assImpl}} 
             &  \multicolumn{2}{c|}{\small Lemma~\ref{lem:Ja_bounded_hessian}}&  {\small Lemma \ref{ass:Ja_estim_bounded_variance}} \\\hline
             \textbf{\textcolor{vibrantRed}{PB Exploration}}  ($\dagger$=P)& $ \cellcolor{brightYellow!30}  \frac{L_p L_\mu R_{\max}}{(1-\gamma)^2} + \frac{ L_r L_\mu }{1 - \gamma} $  & \cellcolor{vibrantMagenta!30} $ \frac{2L_p^2 L_\mu^2 R_{\max}}{(1-\gamma)^3} + \frac{2L_\mu^2L_p L_r+ L_{2,\mu}L_{2,p}R_{\max} }{(1-\gamma)^2} + \frac{L_{2,\mu}L_{2,r}}{1-\gamma}  $ & \cellcolor{vibrantMagenta!30} $ \frac{R_{\max}c (\dt+1)}{\sigma^2_\text{P}(1-\gamma)^2} $  & \cellcolor{vibrantBlue!30} $  \frac{R_{\max} c \dt}{\sigma_{\text{P}}^2(1-\gamma)^2}$ \\\cdashline{2-5}
             {\small \hfill Assumptions:} & {\small \ref{ass:lipMdp}, \ref{ass:lipPol} } & {\small \ref{ass:lipMdp}, \ref{ass:lipPol}, \ref{ass:smoothMdp}, \ref{ass:smoothPol} } & {\small \ref{ass:magic}} & {\small \ref{ass:magic} } \\\cdashline{2-5}
             {\small \hfill Reference:}  & {\small Lemma~\ref{thr:assImpl}} 
             &   \multicolumn{2}{c|}{\small Lemma~\ref{lem:Jp_bounded_hessian}}  &  {\small Lemma~\ref{ass:Jp_estim_bounded_variance}} \\
             \hline
        \end{tabular}
    }
    \caption{Bounds to the Lipschitz and smoothness constants for the AB and PB objectives ($\Ja$ and $\Jp$) and variance of the GPOMDP and PGPE estimators. Both presented bounds on $L_{2,\dagger}$ hold under different sets of assumptions. ${}^\ddagger$ if $\sigma_{\text{A}} < \sqrt{\da}$.}\label{tab:magic}
\end{table*}


% \begin{table*}[t]
%     \centering\renewcommand{\arraystretch}{1.2}
%     \begin{tabular}{|C{2.5cm}|C{2.5cm}|C{2.5cm}|C{2.5cm}|C{2.5cm}|}\hline
%          &  \multicolumn{2}{c|}{Fixed $\sigma$}   &  \multicolumn{2}{c|}{Adaptive $\sigma$} \\ \hline
%          & w/o smoothness & w/ smoothness & w/o smoothness & w/ smoothness  \\ \hline
%          \textbf{\textcolor{vibrantBlue}{GPOMDP}}  & $\frac{\da^2}{\sigma_{\text{A}}^4(1-\gamma)^5\epsilon^3}$ & $\frac{\da}{\sigma_{\text{A}}^2(1-\gamma)^6\epsilon^3}$ & $\frac{\da^4}{(1-\gamma)^{13}\epsilon^7}$ & $\frac{\da^2}{(1-\gamma)^{10}\epsilon^5}$ \\\hline
%          \textbf{\textcolor{vibrantRed}{PGPE}}  &  $ \frac{\dt^2}{\sigma_{\text{P}}^4(1-\gamma)^4\epsilon^3}$ & $ \frac{\dt}{\sigma_{\text{P}}^2(1-\gamma)^5\epsilon^3}$ & $\frac{\dt^4}{(1-\gamma)^{12}\epsilon^7}$ & $\frac{\dt^2}{(1-\gamma)^9\epsilon^5}$ \\
%          \hline
%     \end{tabular}
%     \caption{Caption}\label{tab:convergence}
% \end{table*}

\begin{table}[t]
    \centering\renewcommand{\arraystretch}{1.2}\resizebox{\linewidth}{!}{
    \begin{tabular}{|C{0.3cm}|C{2.2cm}|C{2.5cm}|C{2.5cm}|}\hline
         & & \textbf{\textcolor{vibrantBlue}{GPOMDP}}  & \textbf{\textcolor{vibrantRed}{PGPE}} \\\hline
         \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Fixed $\sigma$}}} & {\small w/o smoothness} & $\displaystyle \frac{\da^2}{\sigma_{\text{A}}^4(1-\gamma)^5\epsilon^3}$ (Theorem~\ref{thr:gpomgp_sam_comp_wgd})  & $\displaystyle \frac{\dt^2}{\sigma_{\text{P}}^4(1-\gamma)^4\epsilon^3}$ (Theorem~\ref{thr:pgpe_sam_comp_wgd})\\ \cline{2-4}
         &  {\small w/ smoothness} & $\displaystyle \frac{\da}{\sigma_{\text{A}}^2(1-\gamma)^6\epsilon^3}$ (Theorem~\ref{thr:gpomgp_sam_comp_wgd}) & $ \displaystyle \frac{\dt}{\sigma_{\text{P}}^2(1-\gamma)^5\epsilon^3}$ (Theorem~\ref{thr:pgpe_sam_comp_wgd})\\ \hline
         \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{$\epsilon$-adaptive $\sigma$}}} & {\small w/o smoothness} & $\displaystyle \frac{\da^4}{(1-\gamma)^{13}\epsilon^7}$ (Theorem~\ref{thr:pg_sam_comp_wgdAdaptive}) & $\displaystyle \frac{\dt^4}{(1-\gamma)^{12}\epsilon^7}$ (Theorem~\ref{thr:pgpe_sam_comp_wgdAdaptive}) \\ \cline{2-4}
         &  {\small w/ smoothness} & $\displaystyle \frac{\da^2}{(1-\gamma)^{10}\epsilon^5}$ (Theorem~\ref{thr:pg_sam_comp_wgdAdaptive}) & $\displaystyle \frac{\dt^2}{(1-\gamma)^9\epsilon^5}$ (Theorem~\ref{thr:pgpe_sam_comp_wgdAdaptive}) \\ \cline{2-4}
         &  {\small w/ smoothness +  inherited WGD} & $\displaystyle \frac{\da^2}{(1-\gamma)^{14}\epsilon^5}$ (Theorem~\ref{thr:gpomgp_sam_comp_wgdInherited}) & $\displaystyle \frac{\dt^2}{(1-\gamma)^{11}\epsilon^5}$ (Theorem~\ref{thr:pgpe_sam_comp_wgdInherited}) \\ \hline
         % & w/o smoothness & w/ smoothness & w/o smoothness & w/ smoothness  \\ \hline
         % \textbf{\textcolor{vibrantBlue}{GPOMDP}}  &  &  &  &  \\\hline
         % \textbf{\textcolor{vibrantRed}{PGPE}}  &  $ & &  & $\frac{\dt^2}{(1-\gamma)^9\epsilon^5}$ \\
         % \hline
    \end{tabular}}
    \caption{Summary of the convergence rates of GPOMDP and PGPE under the various assumptions considered in the paper. \quotes{w/o smoothness} = Assumptions \ref{ass:lipMdp}, \ref{ass:lipPol}, \ref{ass:smoothPol}, \ref{ass:magic}. \quotes{w/ smoothness} = \quotes{w/o smoothness} + Assumption~\ref{ass:smoothMdp}. }\label{tab:convergence}
\end{table}

%\am{In apx, metteiamo anche la concervenza a punto stazionario?}
%\todomp{Non necessario viste le motivazioni, ma per PGPE almeno ci creiamo una reference ad uso futuro. A meno che non vogliamo far vedere che la dipendenza da $\sigma$ e le differenze tra PB e AB valgono anche per FOSP}

\subsection{\textcolor{vibrantRed}{Global Convergence of PB Exploration with PGPE}}\label{sec:globalPGPE}
In this section, we provide the global convergence of PGPE and white noise-based exploration. We start providing the guarantee for \emph{fixed} variance and, then, we move to the \emph{$\epsilon$-adaptive} variance case.\footnote{From now on, the Big-$O$  and Big-$\widetilde{O}$ notations, will retain dependences on $\epsilon$, $(1-\gamma)^{-1}$, $\sigma_{\text{A}}$, $\sigma_\text{P}$, $\dt$, $\da$, and $\alpha$ only.}

\begin{restatable}[\textbf{\textcolor{vibrantRed}{Global convergence of PGPE - Fixed $\sigma_{\text{P}}$}}]{thr}{pgpeSamCompWGD} \label{thr:pgpe_sam_comp_wgd}
     Under Assumptions~\ref{ass:J_wgd} (with $J_{\simbolo}=\Jp$), \ref{ass:lipMdp}, \ref{ass:lipPol}, \ref{ass:magic}, with a suitable constant step size, to guarantee $\Jd^* - \E[\Jd(\vtheta_K)] \le \epsilon + \beta + 3L_J\sqrt{\dt} \sigma_P$, where $3L_J\sqrt{\dt} \sigma_P = O(\sqrt{\dt}\sigma_\text{P}(1-\gamma)^{-2})$ the sample complexity of PGPE is at most:
    \begin{align}
        NK = \widetilde{O} \left( \frac{\alpha^4 \dt^2}{\sigma_{\text{P}}^4(1-\gamma)^4\epsilon^3}\right).
    \end{align}
    Furthermore, under Assumptions~\ref{ass:smoothMdp} and~\ref{ass:smoothPol}, the same guarantee is obtained with a sample complexity at most:
    \begin{align}
        NK = \widetilde{O} \left( \frac{\alpha^4\dt}{\sigma_{\text{P}}^2(1-\gamma)^5\epsilon^3}\right).
    \end{align}
 \end{restatable}

 Some observations are in order. First, the convergence guarantee contains the additional term $3L_J\sqrt{\dt} \sigma_P
$ (depending on $\sigma_{\text{P}}$) that originates from the bound between the objectives $\Jd$ and $\Jp$, as in Section~\ref{sec:deploy}. Second, the sample complexity scales with $\widetilde{O}(\epsilon^{-3})$ for both sets of assumptions. This matches the sample complexity of GPOMDP to converge to the global optimum of $\Ja$ under WGD~\citep[][Cor. 3.7]{yuan2022general}. Third, by enforcing the smoothness of the MDP and of the deterministic policy (Asm.~\ref{ass:smoothMdp} and~\ref{ass:smoothPol}), we improve the dependence on $\dt$ and on 
$\sigma_{\text{P}}$ at the price of an additional $(1-\gamma)^{-1}$ factor. Now, we show that a choice of $\sigma_{\text{P}}$ which adapts to $\epsilon$ allows us to achieve the global convergence on the deterministic objective $\Jd$.

\begin{restatable}[\textbf{\textcolor{vibrantRed}{Global convergence of PGPE - $\epsilon$-adaptive $\sigma_{\text{P}}$}}]{thr}{pgpeSamCompWGDAdaptive} \label{thr:pgpe_sam_comp_wgdAdaptive}
     Under Assumptions~\ref{ass:J_wgd} (with $J_{\simbolo}=\Jp$), \ref{ass:lipMdp}, \ref{ass:lipPol}, \ref{ass:magic}, with a suitable constant step size and {$\sigma_{\text{P}} = \frac{\epsilon}{6L_J\sqrt{\dt}} = O(\epsilon (1-\gamma)^2 \dt^{-1/2})$}, to guarantee $
         \Jd^* - \E[\Jd(\vtheta_K)] \le \epsilon + \beta$ the sample complexity of PGPE is at most:
     \begin{align}
         NK = \widetilde{O} \left( \frac{\alpha^4\dt^4}{(1-\gamma)^{12}\epsilon^7}\right).
 \end{align}
 Furthermore, under Assumptions~\ref{ass:smoothMdp} and~\ref{ass:smoothPol}, the same guarantee is obtained with a sample complexity at most:
          \begin{align}
         NK = \widetilde{O} \left( \frac{\alpha^4\dt^2}{(1-\gamma)^9\epsilon^5}\right).
 \end{align}
 \end{restatable}

We observe that without the smoothness on the MDP and on the deterministic policy (Asm.~\ref{ass:smoothMdp} and~\ref{ass:smoothPol}), the convergence rate becomes $\widetilde{O}(\epsilon^{-7})$ which reduces to $\widetilde{O}(\epsilon^{-5})$ when enforcing them. This better dependence emerges also for $(1-\gamma)^{-1}$ and $\dt$. Clearly, the slower rate of Theorem~\ref{thr:pgpe_sam_comp_wgdAdaptive}, $\epsilon^{-5}$ or $\epsilon^{-7}$, compared to the $\epsilon^{-3}$ of Theorem~\ref{thr:pgpe_sam_comp_wgd} is explained by the more challenging requirement of converging to the \emph{optimal deterministic policy} rather than the \emph{optimal stochastic hyperpolicy}, as for standard PGPE. Note that we have set standard deviation equal to $\sigma_{\text{P}} = \frac{\epsilon}{6L_J\sqrt{\dt}} = O(\epsilon (1-\gamma)^2 \dt^{-1/2})$ that, as expected, decreases with the desired accuracy $\epsilon$. We remark that these results should be interpreted as a demonstration that global convergence to deterministic policies \emph{is possible} rather than a \emph{practical recipe} to set the value of $\sigma_{\text{P}}$. {\color{blue}Nonetheless, we do hope that this theoretical findings can guide the design of practical solutions in future work.}

%\todomp{secondo me dovremmo essere espliciti da subito sul fatto che questi risultati con $\sigma=\epsilon$ non hanno una rilevanza pratica (anche solo per gli evidenti problemi numerici), e puntare sul fatto che mostrano che *è possibile* trovare una policy deterministica $\epsilon$-ottima con un numero polinomiale di sample}
%\am{alla fine però anche i LR teorici dipeendono da epsilon}

\subsection{\textcolor{vibrantBlue}{Global Convergence of AB Exploration with GPOMDP}}\label{sec:globalPG}
We now provide the global convergence of GPOMDP analyzing both fixed and $\epsilon$-adaptive variance choices.

\begin{restatable}[\textbf{\textcolor{vibrantBlue}{Global convergence of GPOMDP - Fixed $\sigma_{\text{A}}$}}]{thr}{gpomdpSamCompWGD} \label{thr:gpomgp_sam_comp_wgd}
      Under Assumptions~\ref{ass:J_wgd} (with $J_{\simbolo}=\Ja$), \ref{ass:lipMdp}, \ref{ass:lipPol}, \ref{ass:smoothPol}, \ref{ass:magic}, with a suitable constant step size, to guarantee $
         \Jd^* - \E[\Jd(\vtheta_K)] \le \epsilon + \beta + 3L\sqrt{\da} \sigma_\text{A}
$, where $3L\sqrt{\da} \sigma_\text{A} = O(\sqrt{\alpha^4\da}\sigma_\text{A}(1-\gamma)^{-2})$ the sample complexity of GPOMDP is at most:
     \begin{align}
         NK = \widetilde{O} \left( \frac{\alpha^4\da^2}{\sigma_{\text{A}}^4(1-\gamma)^5\epsilon^3}\right).
 \end{align}
 Furthermore, under Assumption~\ref{ass:smoothMdp}, the same guarantee is obtained with a sample complexity at most:
          \begin{align}
         NK = \widetilde{O} \left( \frac{\alpha^4\da}{\sigma_{\text{A}}^2(1-\gamma)^6\epsilon^3}\right).
 \end{align}
 \end{restatable}

%\todomp{terrei la dipendenza da $\alpha$: fa vedere che più $\alpha$ è piccolo più la convergenza è veloce}

The result is similar to that of PGPE (Theorem~\ref{thr:pgpe_sam_comp_wgd}) with three notable exceptions. First, an additional $(1-\gamma)^{-1}$ factor appears in the sample complexity due the variance bound of GPOMPD~\citep[][or Table~\ref{tab:magic}]{papini2022smoothing}. This suggests that GPOMDP struggles more than PGPE in long-horizon environments. Second, the dependence on the dimension of the parameter space $\dt$ appearing in Theorem~\ref{thr:pgpe_sam_comp_wgd} gets here replaced with the dimension of the action space $\da$. This is expected and derives from the nature of exploration that is performed in the parameter space for PGPE (PB exploration) and in the action space for GPOMPD (AB exploration). Finally, differently from the PGPE case, the smoothness of the deterministic policy (Asm.~\ref{ass:smoothPol}) is needed for both sample complexity results of GPOMDP.
%the first sample complexity result of Theorem~\ref{thr:gpomgp_sam_comp_wgd} requires an addition to the Lipschizianity of the deterministic policy, its smoothness (Asm.~\ref{ass:smoothPol}). This is necessary to bound the variance of the GPOMDP estimator.
Now, we show that a smart choice of $\sigma_{\text{A}}$ allows us to achieve global convergence on the deterministic objective $\Jd$.

\begin{restatable}[\textbf{\textcolor{vibrantBlue}{Global convergence of GPOMDP - $\epsilon$-adaptive $\sigma_{\text{P}}$}}]{thr}{gpomdpSamCompWGDAdaptive} \label{thr:pg_sam_comp_wgdAdaptive}
   Under Assumptions~\ref{ass:J_wgd} (with $J_{\simbolo}=\Ja$), \ref{ass:lipMdp}, \ref{ass:lipPol}, \ref{ass:smoothPol}, \ref{ass:magic}, with a suitable constant step size and {setting $\sigma_{\text{A}} = \frac{\epsilon}{6L\sqrt{\da}} = O(\epsilon (1-\gamma)^2 \da^{-1/2})$}, to guarantee $\Jd^* - \E[\Jd(\vtheta_K)] \le \epsilon + \beta$ the sample complexity of GPOMDP is at most:
     \begin{align}
         NK = \widetilde{O} \left( \frac{\alpha^4\da^4}{(1-\gamma)^{13}\epsilon^7}\right).
    \end{align}
    Furthermore, under Assumption~\ref{ass:smoothMdp}, the same guarantee is obtained with a sample complexity at most:
    \begin{align}
         NK = \widetilde{O} \left( \frac{\alpha^4\da^2}{(1-\gamma)^{10}\epsilon^5}\right).
    \end{align}
 \end{restatable}

We can notice that the convergence rates display the same dependence on $\epsilon$ as in PGPE (Theorem~\ref{thr:pgpe_sam_comp_wgdAdaptive}) but, the dependence on the effective horizon $(1-\gamma)^{-1}$ is worse.
%Note that the value of $\sigma_{\text{A}} = \frac{\epsilon}{6L\sqrt{\da}} = O(\epsilon (1-\gamma)^2 \da^{-1/2})$, similar to the PGPE case, decreases with the desired accuracy $\epsilon$.

% \am{Non so se di quello sotto serve tenere qualcosa}
% \subsection{Comparison}
% \input{tables/sample_complexity}
% The results presented by Theorems~\ref{thr:pgpe_sam_comp_wgd} and \ref{thr:pg_sam_comp_wgd} show which is the sample complexity $NK$ required by PGPE and GPOMDP when the properties of WGD ($\epsilon' > 0$) or GD ($\epsilon' = 0$) hold for $\Jp$ (PGPE) and $\Ja$ (GPOMDP). 
% We recall that these sample complexities are the ones needed to (approximately) converge to a globally optimal parametrization of the \emph{deterministic} policy $\mu_{\vtheta}$.
% Moreover, we consider the setting in which $\xi_{1} \leq \psigma^{-2}$ and $\upsilon_{1} \leq \asigma^{-2}$.

% Focusing on the dependence on $\epsilon$, $\epsilon'$, and exploration parameters ($\psigma$ and $\asigma$), we can make some comparisons on the sample complexity of the two exploration strategies.
% When the values of $\psigma$ and $\asigma$ are not specified, then in the case in which WGD on $\Jp$ and $\Ja$ holds (\ie $\epsilon' > 0$ and $\delta = \epsilon'$), the sample complexity is $O(\epsilon^{-1} (\epsilon')^{-2} \psigma^{-2})$ for PGPE and $O(\epsilon^{-1} (\epsilon')^{-2} \asigma^{-2})$ for GPOMDP. 
% Conversely, when GD holds on $\Jp$ and $\Ja$ (\ie $\epsilon' = 0$ and $\delta = \epsilon$), we have $O(\epsilon^{-3} \psigma^{-2})$ for PGPE and $O(\epsilon^{-3} \asigma^{-2})$ for GPOMDP.
% Instead, when we set $\psigma$ and $\asigma$ as $O(\epsilon)$, then in the case in which WGD on $\Jp$ and $\Ja$ holds (\ie $\epsilon' > 0$ and $\delta = \epsilon'$), the sample complexity is $O(\epsilon^{-3} (\epsilon')^{-2})$. 
% Conversely, when GD on $\Jp$ and $\Ja$ holds (\ie $\epsilon' = 0$ and $\delta = \epsilon$), we have $O(\epsilon^{-5})$.

% Recovering the additional terms, 
% For generic values of $\psigma$ and $\asigma$, the sample complexity $NK$ is similar form for both the algorithms.
% Notice that the sample complexities of the two algorithms show the trade-off that we already observed in Section~\ref{sec:deploying_det_pol}.
% Indeed, the sample complexity of PGPE depends on the number of parameters $\dt$ employed by the hyperpolicy $\nu_{\vtheta}$ (and by the deterministic policy $\mu_{\vtheta}$).
% On the other hand, the sample complexity of GPOMDP depends on the action dimensionality $\da$ and, moreover, it suffers (more than PGPE) from large task horizons.  \todomp{quantificare}

% Notice that, for a fixed (hyper)policy variance, the $O(\epsilon^{-3})$ convergence is up to a variance-dependent error term.
% This is because we are studying the convergence to a globally optimal deterministic policy, and not the to the optima of the surrogate functions optimized by AB and PB.
% The added difficulty explains why, once we select the (hyper)policy variance to optimize the trade-off between convergence speed and quality of the final solution, the sample complexity is $O(\epsilon^{-5})$.

% \am{Commento sulla dipendenza dall'orizzonte}
% \am{Un'altra cosa che non si evidenzia è la necessità o meno di avere $\mu$ lipshitz/smooth}
% \ale{lo metto dopo in sez 5 quando si caratterizzano L e Lj}

% \am{Qua si potrebbe far riferimento alle proprietà del noise:
% $$
%     \E_{\vtheta' \sim \nu_{\vtheta}} [ \| \nabla_{\vtheta} \log \nu_{\vtheta}(\vtheta') \|_2^2 ] = \E_{\vepsilon \sim \Phi} [ \| \nabla_{\vepsilon} \log \phi(\vepsilon) \|_2^2 ]
% $$
% Non saprei se si riesce a semplificare ulteriormente. Un'osservazione (Cramér–Rao bound):
% \begin{align}
%     & \mathbf{0} = \E_{\vepsilon \sim \Phi}[\vepsilon] \implies \\
%     & \mathbf{0}_{\text{matrix}} = \nabla_{\vepsilon} \E_{\vepsilon \sim \Phi}[\vepsilon] = \E_{\vepsilon \sim \Phi}[\nabla_{\vepsilon} \log \phi(\vepsilon)\vepsilon^\top] + \mathbf{I} \\
%     &  \implies 0\ge - \sqrt{\E_{\vepsilon \sim \Phi}[\|\nabla_{\vepsilon} \log \phi(\vepsilon)\|_2^2]\E_{\vepsilon \sim \Phi}[\|\vepsilon\|_2^2]} + 1\\
%     & \implies  {\E_{\vepsilon \sim \Phi}[\|\nabla_{\vepsilon} \log \phi(\vepsilon)\|_2^2] }\ge (d\sigma^2)^{-1}
% \end{align}
% }
